Equivariant decomposition of polynomial vector fields

To compute the unique formal normal form of families of vector fields with nilpotent linear part, we choose a basis of the Lie algebra consisting of orbits under the linear nilpotent. This creates a new problem: to find explicit formulas for the structure constants in this new basis. These are well known in the 2D case, and recently expressions were found for the 3D case by ad hoc methods. The goal of the present paper is to formulate a systematic approach to this calculation. We propose to do this using a rational method for the inversion of the Clebsch-Gordan coefficients. We illustrate the method on a family of 3D vector fields and compute the unique formal normal form for the Euler family both in the 2D and 3D case.

==> STCOintro.tex <==
\def\sad{{\rm ad}}
\def\mf{\mathfrak}
\section{Introduction}\label{sec:1}
	In \cite{baider1992further} the following problem was addressed: Consider formal vector fields in  \(\mathbb{R}^2\) with a fixed nilpotent linear part \(N\).
For each such vector field, determine the unique normal form, that is a form in which the vector field can be transformed by formal transformations such that the only transformations that are still possible without perturbing the normal form choice are symmetries of the vector field.
		
This was done by constructing a new basis for the formal vector fields in such a way if \(v_i\) is a basis vector, so is \(v_{i+1}=\sad_N v_i\).
The inversion of \(\sad_N\) is then a simple matter of changing the appropriate index from \(i\) to \(i-1\), if \(i>0\).
This we call equivariant decomposition of the vector fields.

In this paper we aim to generalize this procedure from \(\mathbb{R}^2\) to \(\mathbb{R}^n\).
Before the reader gets too excited about this, we should point out that we do not aim to solve the unique normal form problem for \(n\)-dimensional nilpotent systems.
The fact that even the \(2\)-dimensional results are not complete may give an indication of the size of such an undertaking.
What we want to obtain here is an explicit way to compute the structure constants in a basis given by orbits of the nilpotent.

One might ask, why go to the \(3\)-dimensional case if the \(2\)-dimensional case is not done yet. To give at least a partial response to this question
we analyze a \(2\)-dimensional case, the Eulerian vector fields, that was left open in loc. cit., in Section \ref{2DBT}. 
We will see that the \(3\)-dimensional result is very similar to the \(2\)-dimensional result. This is a phenomenon that is familiar from Classical Invariant Theory.
One can expect that the \(4\)-dimensional analysis will be much harder (but then the \(5\)-dimensional case should be similar to the \(4\)-dimensional).

The complexities of this programme are already clear in the treatment of the \(3\)-dimensional irreducible nilpotent singularity in \cite{JF2019vector}.
There the structure constants are computed using Maple computations and extrapolation, a time consuming method which does not seem to be well suited for higher dimensions.
In this paper we will formulate a procedure to compute the structure constants using two ideas:
\begin{itemize}
\item
Use the Clebsch-Gordan coefficients to express two-tensors in terms of \(N\) orbits of transvectants and apply this both in the symmetrical case to products of functions and in the
antisymmetrical case to Lie brackets.
\item
Compute the transvectants, using the fact that we know how to express them using a Stanley basis \cite[Chapter 12]{SVM2007}.
This last condition restricts at the moment the dimension \(n\) to be less than \(6\), at least in the irreducible case.
\end{itemize}
We hope that these techniques will enable the computation of the structure constants for the basis of \(N\)-orbits for higher dimensions,
although we realize that this will probably need some more ideas in order to be completely carried out (the difficulty being the lack of explicit formulas for the transvectants).
We mention here that if one is only interested in carrying out this program for finite jet degree, there should be no difficulty in higher dimensions; it is the infinite dimensional character
of the the problem and our need for explicit formulas that is causing the difficulties.

For the moment the \(3\)-dimensional programme of computing the unique normal form with nilpotent singularity will keep us busy for a while, if the experience with the \(2\)-dimensional
case, were there are still subcases that are not completely understood, is any indication.

The first step is to construct an \(\mathfrak{sl}_2\)-triple \(\langle N, H, M\rangle\), where \(H\) and \(M\) are also linear vector fields, using the Jacobson-Morozov Lemma (see \cite{knapp2013lie,collingwood1993nilpotent}). This triple is not uniquely determined, and one can possibly make choices here that are most suitable for the given situation.
This construction is possible when the linear vector fields form a reductive Lie algebra, as is the case for \(\mf{gl}_n\) and \(\mf{sp}_n\).

\def\im{\mathrm{im}\ }
A vector field is said to be in {\em first level normal form} if its nonlinear part is contained in \(\ker \sad_M\).
The reason for this is that the finite dimensional representation theory of \(\mathfrak{sl}_2\) teaches us that a finite dimensional \(\mathfrak{sl}_2\)-module \(V\) is isomorphic (as modules, not as Lie algebras) to  \(\im \sad_N\oplus\ker \sad_M\).

The next step is to define a basis of vector fields of a given degree \(d\) by first giving a basis for the elements in \(\ker\sad_M\) of that degree, say \(\{v^{d,1},\cdots,v^{d,k}\}\) 
	and then adding to the general basis the elements \(v^{d,i}_k=\sad_N^k v^{d,i}, i=1,\cdots,k, k=1,\cdots,\infty\).
Despite the \(\infty\) in this definition, this is a finite set due to the nilpotent character of \(N\).
This way, it is easy to see what the preimage under \(\sad_N\) is, but the problem is now that one does not have immediately explicit formulas for the structure constants of the Lie algebra with this basis.
%The lack of explicit expressions makes it difficult to rely on the usual tools of Lie algebras, as for instance the Killing form.
\iffalse
\begin{rem}
(JS) I would like to have a basis that is build from a number of commuting vector fields in \(\ker\ad_M\), which are then multiplied with suitable subrings of \(\ker L_M\) to
obtain the whole of \(\ker\sad_M\). Think of powers of the matrix of \(M\).
I do not see how to connect this to the description in \cite{SVM2007}.
The powers of \( M \) seem to be related to transvectants of \(\mathfrak{a}\) and \(\mathfrak{u}\).
\end{rem}
Vector fields are of the form \(\sum_{\alpha,i} v_{\alpha,i} \mathbf{x}^\alpha \frac{\partial}{\partial x_i}\), where \(\alpha\) is a multiindex with the dimension of the underlying vector space.
First of all, we determine \(\mathbb{R}\)-linear combinations \(\sum_j w_j \frac{\partial}{\partial x_j}\) that commute with \(M\).
Let us call them \(\mathfrak{u}_k, k=1,\cdots, u_M\).
Next we determine the generators of the ring \(\ker L_M\). This gives us a finite list, say \(\mathfrak{a}_k, k=1,\cdots, p_M\).
Taking transvectants, one can now find generators \(\mathfrak{v}_1,\cdots,\mathfrak{v}_{v_M}\) of the \(\ker L_M\)-module \(\ker \ad_M\).
A general element in \(\ker\ad M\) can be written as 
\(\sum_{i=1}^{v_M} F_i(\mathfrak{a}_{i^i_1},\cdots,\mathfrak{a}_{i^i_{p_i}}) \mathfrak{v}_i\), 
where the \(i^i_j\) are an \(i\)-dependent subset of \(\{1,\cdots,p_M\}\), the Stanley decomposition of \(\ker\sad_M\).
\begin{question}
Are the \(\mathfrak{v}_i\) commuting?
My guess would be that the vectors at the same transvectant level (like \((\mathfrak{a},\mathfrak{u)}^{(1)}\) and \((\mathfrak{b},\mathfrak{u})^{(1)}\))
generate a subalgebra.
\end{question}
\fi
\iffalse
Explicit Stanley decompositions (that is, descriptions of a basis for \(\ker\sad_M\)), are known for dimension less than six, cf. \cite[Chapter 12]{SVM2007}.
For higher dimensions the  syzygy problems from Classical Invariant Theory make things too difficult to handle (sofar).
\begin{exm}
We consider the \(3\)-dimensional equations with irreducible nilpotent \(N=x\frac{\partial}{\partial y} + 2y  \frac{\partial}{\partial z}\).
Then \(M=2z\frac{\partial}{\partial y}+y\frac{\partial}{\partial x}\) and \(H=2z\frac{\partial}{\partial z}-2x\frac{\partial}{\partial x}\).(CHECK)
Then \(\ker\ad_M\) is \(F_A(z,\Delta) E\mathbf{x}+F_B(z,\Delta) M\mathbf{x} +F_C(z,\Delta)M^2\mathbf{x}\), where \(\Delta=xz-y^2\), \(E=x\frac{\partial}{\partial x}
+y\frac{\partial}{\partial y}+z\frac{\partial}{\partial z}\) and \(\mathbf{x}=\begin{pmatrix}x\\y\\z\end{pmatrix}\).
REMARK Missing here is \((1,0,0)\).
This leads naturally to a direct sum decomposition of Lie subalgebras.
Consider the \(\mathcal{A}\)-family, of vector fields of type
\[
N+F(\mathbf{x}) E.
\]
One defines a basis by \(v^{i,m,n}=\ad_N^i z^m \Delta^n E=(N^i z^m) \Delta^n E\). Then \(\ad_N v^{i,m,n}=v^{i+1,m,n}\)
and \([v^{i,m,n},v^{j,p,q}]=((N^i z^m) \Delta^n (p+2q) (N^j z^p) \Delta^q  -(N^j z^p) \Delta^q (m+2n) (N^i z^m) \Delta^n) E \)
and this equals \((p+2q-m-2n) \Delta^{n+q} (N^i z^m) (N^j z^p) E\).
The product \( (N^i z^m) (N^j z^p) \) is a typical example of an expression that can be analyzed using Clebsch-Gordan coefficients.
\begin{thm}[Rational Clebsch-Gordan Coefficients]

Define  
the \(3j\)-symbol 
\[\begin{pmatrix} m& n& m+n-2p\\i&j& k\end{pmatrix}=\frac{i!j!}{k!}\sum_{r=0}^k (-1)^{i-r}\binom{m-i+r}{m-p}\binom{n+i-r-p}{n-p}\binom{k}{r}, \]
with \(j_1=m, j_2=n\) and \(j_3=n+m-2p\) as the \(3j\)'s. 
The general formula is
\bas
v^{(m)}_i\otimes v^{(n)}_j&=&\sum_{p+k=i+j}\begin{pmatrix} m&n&m+n-2p\\i&j&k\end{pmatrix}\frac{ \binom{m}{i}\binom{n}{j}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes v^n.
\eas
\end{thm}
We will show that
                                \( \Join^{2(p+q-2n)}z^p\otimes z^q=z^{p+q-2n}\Delta^n(2n)!
	\left( n! \right) ^{2}{2\,n-p-q-1\choose n} {n-p-1\choose n}{n-q-1
	\choose n}
\)
\end{exm}
One defines the comultiplication \(\Delta\) by
\ba 
\Delta(X)&=&X\otimes 1+1\otimes X 
\ea
Suppose now we have two elements \(v^m\) and \(w^n\) in \(\ker\sad_M\). Suppose the have \(\sad_H\)-eigenvalues \(m, n\), respectively.
We write \(v_{i}^{m}=\sad_N^i v^m, i=0,\ldots,m\).
We now want an explicit formula of the Lie bracket of \(v_{i}^{m}\) and \(w_{j}^{n}\) in terms of transvectants of \(v^m\) and \(w^n\).
What are transvectants? They are formulas for the projections described in the Clebsch-Gordan formula
\[
V_{m}\otimes V_{n}=\bigoplus_{p=0}^{\min(m,n)} V_{m+n-2p},
\]
where \(V_{m}=\langle \sad_N^k
v^{m}\rangle_{k=0,\ldots,m}
\), and the projections \(\Join^{m+n-2p}: V_{m}\otimes V_{n}\rightarrow V_{m+n-2p}\cap \ker\Delta(\sad_{M})\) (that is, \(V_{m+n-2p}=\langle \Join^{m+n-2p}_k v^{m}\otimes w^{n}= \Delta^k(\sad_{N})
\Join^{m+n-2p} v^{m}\otimes w^{n}\rangle\rangle_{k=0,\ldots,m+n-2p}\))  are given by
\[
\Join^{m+n-2p} v^{m}\otimes w^{n}=
			p! \sum_{i+j=p}(-1)^i\binom{ m-i}{p-i}  \binom{n-j}{p-i}v_{i}^{m}\otimes w_{j}^{n},\quad p\leq\min(m,n).
\]
There is a corresponding bracket
\[
[ v^{m}, w^{n}]^{({m+n-2p})}=
			p! \sum_{i=0}^p(-1)^i{ {m-i}\choose{p-i}}  { {n-p+i}\choose{i}}[v_{i}^{m}, w_{p-i}^{n}],\quad p\leq\min(m,n).
\]
The \(p\)th transvectant is an element of \(\ker \Delta(\sad_{M})\) with \(\Delta(\sad_H)\)-eigenvalue \(m+n-2p\), and the corresponding bracket is an element of \(\ker\sad_M\) with \(\sad_H\)-eigenvalue \(m+n-2p\).
%that is \[
%V_{\omega_v+\omega_w-2k}=
%\langle \sad_N^r \pi^k v^{0}_{\omega_v}\otimes w^{0}_{\omega_w} \rangle_{r=0,\ldots,\omega_v+\omega_w-2k}
%=
%\langle \sad_N^r [ v^{0}_{\omega_v}, w^{0}_{\omega_w}]^{(k)} \rangle_{r=0,\ldots,\omega_v+\omega_w-2k}
%\]
\begin{rem}
The term {\em transvectant} brings us back to Classical Invariant Theory. It has been superseded by more general construction methods that work for general Lie algebras.
But in normal form theory the only nonabelian Lie algebra one encounters is \(\mathfrak{sl}_2\), so there is no need to go to such generality for us.
Transvectants have a way of showing up in unexpected places. This is a manifestation of {\em hidden symmetry}.
\end{rem}
The formula we aim at is of the form
\[
v_{i}^{m}\otimes w_{j}^{n}=\sum_{p+k=i+j}\alpha_{i,j,k}^{m,n,m+n-2p}
{\Join_k^{m+n-2p} v^{m}\otimes w^{n}}
\]
or
\[
[v_{i}^{m}, w_{j}^{n}]=\sum_{k+p=i+j} \alpha_{i,j,k}^{m,n,m+n-2p}
{\sad_N^{k}[ v^{m}, w^{n}]^{(n+m-2p)}}
\]
Formulas like this are well known in the literature:
One defines the \(3j\)-symbol implicitly by
\[
{\Join^{m+n-2p}_k v^{m}\otimes w^{n}}
=\sum_{i+j=p+k}\left(\begin{array}{ccc} m &n & m+n-2p\\ i&j&k\end{array}\right)v_{i}^{(m)} \otimes v_{j}^{(n)}.
\]
\begin{rem}
Different conventions apply. Watch the difference between \(v_i^m\) and \(v_i^{(m)}\).
\end{rem}
\fi
\iffalse
Then one can express the \(\alpha\)s in terms of the \(3j\)-symbols.
%The problem with this approach for us is that there is no general explicit formula for the \(3j\)-symbols. 
%The approach works fine for given numbers, but not in the generality that we would like to obtain.
Since we could find nothing that we could use in the literature, apart from remarks that such explicit formulas did not exist, we formulated and proved
the following
\begin{thm}
Let \(v,w\in\ker\sad_M\) with \(\sad_H\)-eigenvalues \(m,n\), respectively. Then
\ba \label{TF1}
[\sad_N^r v,w]=\sum _{k+p=r} (-1)^p \binom{r}{p} {\frac { \left( n+m-2\,p+1 \right)  \prod _{i=p}^{r-1}(m-i)}{ \prod _{i=-1}^{r-1}(m+n-i-p)}} \sad_N^{k} [v^m,w^n]^{(n+m-2p)}.
\ea
where
\(\omega_{vw}=\omega_v+\omega_w.\)
\end{thm}
\begin{rem}
Notice that 
\[
\prod _{i=-1}^{r-1}(m+n-i-p)=\prod _{i=0}^{r}(m+n-i+1-p)=\binom{m+n+1-p}{r+1}(r+1)!
\]
\end{rem}
This leads to explicit formulas for \([\sad_N^k v,\sad_N^l w]\) and allows us to determine the structure constants for the Lie algebra of polynomial vector fields.
\begin{rem}
There is a potential problem with the contraction. Even if a tensor \(v\otimes w\) is nonzero, the bracket may well be zero.
\end{rem}
A problem with the bracket transvectants is that they are computed using the brackets that we would like to be able to compute.
Is it possible to predict what they will be on the basis of their degrees and eigenvalues, if we have a complete description of the kernel of \(\sad_M\)?
In the present formulation, the kernel of \(\sad_M\) is described as a \(\ker\L_M\)-module.
Is it possible to describe it as a \(\ker\sad_M\)-module, with transvection as the action?
\fi
\iffalse
\section{Some computations}
Let \(f,g\in\ker M\).
\bas
[\sad_N^n fM ,gM]&=&
\sum _{k=0}^{n} (-1)^k \binom{n}{k} {\frac { \left( \omega_{fg}-2\,k+5 \right)  \prod _{i=k}^{n-1}(\omega_{{f}}-i+2)}{ \prod _{i=-1}^{n-1}(\omega_{fg}-i-k+4)}} \sad_N^{n-k} [fM,gM]^{(k)}
\eas
We now have to show that \([fM,gM]^{(k)}=hM\). This does not seem to be obvious.
\bas
[\ad_N fM,gM]&=&[N(f)M-fH,gM]
\\&=&-g MN(f) M -(\omega_g+2) fg M
\\&=& -(\omega_{fg}+2) f g M
\eas
\bas
[\ad_N^2 fM,gM]&=&[\ad_N (N(f)M-fH),gM]
\\&=&[N^2(f) M -2 N(f)H- 2 fN,GM]
\\&=& 
\eas
%\iffalse
\section{Quantum groups}
We define \(U_q = U_q(\mathfrak{sl}_2) \) as the algebra generated by
the four variables \(M, N, K, K^{- 1}\) with the relations
\bas
KK^{- 1}&=& K^{-1}K\\
KM&=& q^2MK,\quad KN= q^{- 2}NK,
\eas
and
\bas
[M,N]&=&\frac{K^2 - 1}{ q^2 - 1}
\eas
Let \(v_a^0\in\ker M\), with \(K v_a^0=q^a v_a^0\).
Then let \(v^j_a=N^j v^0_a\).
We find \(K v^j_a=K N^j v^0_a=q^{-2j} N^j K v^0_a= q^{a-2j} v^j_a\).
\iffalse
Let
\[
\begin{array}{ccc} Mv^i_m=[i][m-i+1] v^{i-1}_m &  N v^{i-1}_m=v^i_m & Kv^i_m=q^{m-2i} v^i_m\\
\end{array}
\]
\fi
%Then \(\pi^0_q v^0_1\otimes v^0_1=v^0_1\otimes v^0_1\) and \(\pi^1_q v^0_1\otimes v^0_1= v^1_1 \otimes v^0_1-q v^0_1 \otimes v^1_1\).

One defines the comultiplication \(\Delta\) by
\ba 
\Delta(N)&=&N\otimes 1+1\otimes N \\
\Delta(M)&=&M\otimes K^2+1\otimes M\\
\Delta(K)&=&K\otimes K\\
\Delta(1)&=&1\otimes 1
\ea
\begin{lem}
\[
\Delta(K)\Delta(N)=q^{-2}\Delta(N)\Delta(K).
\]
\end{lem}
\begin{proof}
\bas
\Delta(K)\Delta(N)&=& K\otimes K(N\otimes 1+1\otimes N)
\\&=& KN\otimes K+K\otimes KN
\\&=& q^{-2}(NK\otimes K+K\otimes NK)
\\&=& q^{-2}(N\otimes 1+1\otimes N)K\otimes K
\eas
\end{proof}
\begin{lem}
\[
\Delta(K)\Delta(M)=q^2\Delta(M)\Delta(K).
\]
\end{lem}
\begin{proof}
\bas
\Delta(K)\Delta(M)&=&K\otimes K (M\otimes K^2+1\otimes M)
\\&=&KM\otimes K^3+K\otimes KM
\\&=&q^2 (MK\otimes K^3+K\otimes MK)
\\&=&q^2 (M\otimes K^2+1\otimes M)K\otimes K
\\&=&q^2 \Delta(M)\Delta(K).
\eas
\end{proof}
\begin{lem}
\[
[\Delta(M),\Delta(N)]=\frac{\Delta(K)^2-\Delta(1)}{q^2 - 1}.
\]
\end{lem}
\begin{proof}
\bas
[\Delta(M),\Delta(N)]&=&(M\otimes K^2+1\otimes M)(N\otimes 1+1\otimes N)-(N\otimes 1+1\otimes N)(M\otimes K^2+1\otimes M)\\
&=&[M,N]\otimes K^2+1\otimes [M,N]\\
&=&\frac{K^2 -  1}{ q^2 - 1}\otimes K^2+1\otimes \frac{K^2 - 1}{ q^2 - 1}\\
&=&\frac{K^2 \otimes K^2}{ q^2 - 1}-\frac{1\otimes 1}{ q^2 - 1}=\frac{\Delta(K)^2-\Delta(1)}{q^2 - 1}.
\eas
\end{proof}
Let \((n)_q=\frac{q^{2n}-1}{q^2-1}\) and
\(v^{(i)}_m=\frac{1}{(i)_q} v^i_m\). Notice that \(\lim_{q\downarrow 0} (n)_q=1\) and \(\lim_{q\rightarrow 1} (n)_q=n\).
\bas
\pi^s_q v_a\otimes v_b& =&\sum_{i+j=s} (-1)^j q^{j(b-j+1)} \frac{(a-i)_q!(b-j)_q!}{(a-s)_q!(b-s)_q!}  v^{(i)}_a \otimes {v}^{(j)}_b
\\& =&\sum_{i+j=s} (-1)^i q^{j(b-j+1)}  \frac{(a-i)_q!(b-j)_q!}{(a-s)_q!(j)_q!(b-s)_q!(i)_q!}  v^{i}_a \otimes {v}^{j}_b
\\& =&\sum_{i+j=s} (-1)^i q^{j(b-j+1)}  \binom{a-i}{s-i}_q\binom{b-j}{s-j}_q  v^{i}_a \otimes {v}^{j}_b
\eas
\begin{defn}
Let \((K;n)=\frac{K^2 q^{2n}-1 }{q^2-1}\). 
%\([K;a]=\frac{K q^a- K^{-1} q^{-a}} {q-q^{-1}}\)
\end{defn}
\begin{lem}
\((K;n)N=N(K;n-2)\)
\end{lem}
\begin{proof}
\bas
(K;n)N&=&\frac{K^2 q^{2n}-1 }{q^2-1}N
\\&=&N\frac{K^2 q^{2n-4}-1 }{q^2-1}
\\&=&N(K;n-2)
\eas
\end{proof}
\begin{lem}
\([M,N^k]=(k)_q N^{k-1}(K;1-k)
\).
		\end{lem}
\begin{proof}
For \(k=1\) the statement is \([M,N]=(1)_q (K;0)=\frac{K^2 -1 }{q^2-1}\), which is true by the definition of \(U_q(\mathfrak{sl}_2)\).
Then we use induction with respect to \( k\) to show that
\bas
[M,N^{k+1}]&=&MN^k N - N^{k+1} M
\\&=& N^kM N + (k)_q N^{k-1}(K;1-k)N - N^{k+1} M
\\&=&  N^k (K;0) + (k)_q N^{k}(K;-1-k) 
\\&=& \frac{N^k}{(q^2-1)^2} \left\{ K^2q^2 -K^2  -q^2+ 1  + (q^{2k}-1) (K^2 q^{-2(1+k)} -1)\right\}
\\&=& \frac{N^k}{(q^2-1)^2} \left\{ K^2q^2 -K^2  -q^2+ 1  + K^2 q^{-2} -K^2 q^{-2(1+k)} -q^{2k}+1 )\right\}
\\&=& \frac{N^k}{(q^2-1)^2} \left\{ K^2(q^2 - 1) -(q^2- 1)  + K^2 q^{-2} -K^2 q^{-2(1+k)} -q^{2k}+1 )\right\}
\eas
\end{proof}
\bas
[M,N^{2}]&=&MN N - N^2 M
\\&=& [M,N]N +N [M,N]
\\&=& \frac{K^2 -1 }{q^2-1}N +N \frac{K^2 -1 }{q^2-1}
\\&=& \frac{N}{q^2-1}(K^2q^{-4} -1 + K^2 -1 )
\eas
\bas
(2)_q N(K;-1)&=&\frac{q^4-1}{q^2-1} N \frac{K^2 q^{-2}-1 }{q^2-1}
\\&=&N (q^2+1)  \frac{K^2 q^{-2}-1 }{q^2-1}
\\&=&\frac{N}{q^2-1}  (K^2 q^{-2}-1+K^2-q^2 )
\eas
XXX
\begin{cor}
\(M v^k_a=[k][a+1-k] v^{k-1}_a\)
\end{cor}
\begin{proof}
\(M v^k_a=[k] N^{k-1}[K;1-k] v^0_a=[k] N^{k-1} \frac{ q^{a+1-k}- q^{-a+k-1}}{q-q^{-1}}v^0_a=[k][a+1-k] v^{k-1}_a\)
\end{proof}
\begin{lem}
\([M,(NK)^k]=[k] (NK)^{k-1}[K;1-k] K
\).
		\end{lem}
\begin{proof}
Let \(k=1\). Then \([M,NK]=MNK-NKM=[K;0] K +NMK-NKM=[K;0] K +q^{-2} NKM-NKM\)
Let \(v_m\in\ker_M\). Then \([M,NK]v_m=MNK v_m=MN q^m v_m=[M,N] q^m v_m =[K;0] q^m v_m=[K;0]K v_m\).
Then we use induction with respect to \( k\) to show that
\bas
[M,(NK)^{k+1}]&=&M(NK)^k  NK - (NK)^{k+1} M
\\&=& (NK)^kM NK + [k](NK)^{k-1}[K;1-k]KNK  - (NK)^{k+1} M
\\&=& (NK)^k[K;0]K +(NK)^k NM K  + [k] (NK)^{k-1}KN[K;-1-k]K  - (NK)^{k+1} M
\\&=& (NK)^k[K;0]K +(NK)^k K  NM  + [k] (NK)^{k-1}KN[K;-1-k]K  - (NK)^{k+1} M
\\&=& (NK)^k[K;0]K   + [k] (NK)^{k}[K;-1-k]  K
\\&=& [k+1] (NK)^k [K;-k]K.
\eas
\end{proof}
\begin{thm}
If \(v_a\otimes v_b\in \ker\Delta(M)\), then \(\pi^s_q v_a\otimes v_b\in \ker\Delta(M)\).
\end{thm}
\begin{proof}
\bas
\Delta(M) \pi^s_q v_a\otimes v_b&=& \sum_{i+j=s} (-1)^i q^{j(b-j+1)} \binom{a-i}{s-i}\binom{b-j}{s-j}  M  v^{i}_a \otimes K {v}^{j}_b\\&&
+\sum_{i+j=s} (-1)^i q^{j(b-j+1)} \binom{a-i}{s-i}\binom{b-j}{s-j}  v^{i}_a \otimes M {v}^{j}_b
\\&=& \sum_{i+j=s} (-1)^i q^{j(b-j+1)} \frac{[a-i]![b-j]!}{[a-s]![b-s]![j]![i]!} [i][a+1-i]  v^{i-1}_a \otimes q^{b-2j} {v}^{j}_b\\&&
+\sum_{i+j=s} (-1)^i q^{j(b-j+1)} \frac{[a-i]![b-j]!}{[a-s]![b-s]![i]![j]!}   v^{i}_a \otimes  [j][b+1-j] {v}^{j-1}_b
\\&=& \sum_{i+j=s} (-1)^i q^{(j+1)(b-j)} \frac{[a-i+1]![b-j]!}{[a-s]![b-s]![j]![i-1]!}   v^{i-1}_a \otimes {v}^{j}_b\\&&
+\sum_{i+j=s} (-1)^i q^{j(b-j+1)} \frac{[a-i]![b+1-j]!}{[a-s]![b-s]![i]![j-1]!}   v^{i}_a \otimes  {v}^{j-1}_b
\\&=&-\sum_{i+j=s-1} (-1)^i q^{(j+1)(b-j)} \frac{[a-i]![b-j]!}{[a-s]![b-s]![j]![i]!}   v^{i}_a \otimes {v}^{j}_b\\&&
+\sum_{i+j=s-1} (-1)^i q^{(j+1)(b-j)} \frac{[a-i]![b-j]!}{[a-s]![b-s]![i]![j]!}   v^{i}_a \otimes  {v}^{j}_b
\\&=&0.
\eas
\end{proof}
\begin{rem}
(JS, 26-1-2019) If we replace \(q^{j(b-j+1)}N^j\) by \((NK)^j\) I can not get the proof to work. After applying \(M\) I end up with an extra \(K\).
\end{rem}
Let us MMM check whether this is compatible with the earlier definitions.
\bas
\pi^1_q v_a\otimes v_b& =& \sum_{i+j=1} (-1)^i q^{j(b-j+1)}  \binom{a-i}{1-i}\binom{b-j}{1-j}  v^{i}_a \otimes {v}^{j}_b
\\&=& q^{b}  \binom{a}{1}\binom{b-1}{0}  v^{0}_a \otimes {v}^{1}_b
-  \binom{a-1}{0}\binom{b}{1}  v^{1}_a \otimes {v}^{0}_b
\\&=& q^{b}  [a]  v^{0}_a \otimes {v}^{1}_b
-  [b]  v^{1}_a \otimes {v}^{0}_b
\eas
The limit for \(q\rightarrow 1\) seems fine, but for \(q\rightarrow 0\) not.
\iffalse
\bas
\pi^1_q v_a\otimes v_b& =&
\sum_{\alpha=0}^1 (-1)^\alpha q^{(1-\alpha)(\alpha+1)} \left( \prod_{\beta=1}^\alpha \frac{q^{2(b-1+\beta)}-1}{q^{2(a-\beta+1}-1} \right) v^{(\alpha)}_a \otimes v^{(1-\alpha)}_b\\
&=&
q v^{(0)}_a \otimes v^{(1)}_b-
\left(  \frac{q^{2b}-1}{q^{2a}-1} \right) v^{(1)}_a \otimes v^{(0)}_b\\
\eas
\fi
\fi
\iffalse
\section{Quantum groups}
We define \(U_q = U_q(\mathfrak{sl}_2) \) as the algebra generated by
the four variables \(M, N, K, K^{- 1}\) with the relations
\bas
KK^{- 1}&=& K^{-1}K\\
KM&=& q^2MK,\quad KN= q^{- 2}NK,
\eas
and
\bas
[M,N]&=&\frac{K - K^{- 1}}{ q - q^{-1}}
\eas
Let \(v_a^0\in\ker M\), with \(K v_a^0=q^a v_a^0\).
Then let \(v^j_a=N^j v^0_a\).
We find \(K v^j_a=K N^j v^0_a=q^{-2j} N^j K v^0_a= q^{a-2j} v^j_a\).
\iffalse
Let
\[
\begin{array}{ccc} Mv^i_m=[i][m-i+1] v^{i-1}_m &  N v^{i-1}_m=v^i_m & Kv^i_m=q^{m-2i} v^i_m\\
\end{array}
\]
\fi
%Then \(\pi^0_q v^0_1\otimes v^0_1=v^0_1\otimes v^0_1\) and \(\pi^1_q v^0_1\otimes v^0_1= v^1_1 \otimes v^0_1-q v^0_1 \otimes v^1_1\).

One defines the comultiplication \(\Delta\) by
\ba 
\Delta(N)&=&N\otimes 1+K^{-1}\otimes N \\
\Delta(M)&=&M\otimes K+1\otimes M\\
\Delta(K)&=&K\otimes K
\ea
\begin{lem}
\[
\Delta(K)\Delta(M)=q^2\Delta(M)\Delta(K).
\]
\end{lem}
\begin{proof}
\bas
\Delta(K)\Delta(M)&=&K\otimes K (M\otimes K+1\otimes M)
\\&=&KM\otimes K^2+K\otimes KM
\\&=&q^2 (MK\otimes K^2+K\otimes MK)
\\&=&q^2 (M\otimes K+1\otimes M)K\otimes K
\\&=&q^2 \Delta(M)\Delta(K).
\eas
\end{proof}
\begin{lem}
\[
[\Delta(M),\Delta(N)]=\frac{\Delta(K)-\Delta(K)^{-1}}{q - q^{-1}}.
\]
\end{lem}
\begin{proof}
\bas
[\Delta(M),\Delta(N)]&=&(M\otimes K+1\otimes M)(N\otimes 1+K^{-1}\otimes N)-(N\otimes 1+K^{-1}\otimes N)(M\otimes K+1\otimes M)\\
&=&[M,N]\otimes K+K^{-1}\otimes [M,N]\\
&=&\frac{K - K^{- 1}}{ q - q^{-1}}\otimes K+K^{-1}\otimes \frac{K - K^{- 1}}{ q - q^{-1}}\\
&=&\frac{K \otimes K}{ q - q^{-1}}-\frac{K^{-1}\otimes K^{- 1}}{ q - q^{-1}}=\frac{\Delta(K)-\Delta(K)^{-1}}{q - q^{-1}}.
\eas
\end{proof}
\iffalse
Then let \bas
v^0_1\otimes v^1_1&=&\alpha_{011}^{111}(\pi^1_q v^0_1\otimes v^0_1) + \alpha_{010}^{111} \Delta(N) \pi^0_q v^0_1\otimes v^0_1\\
&=& \alpha_{011}^{111}(v^1_1 \otimes v^0_1-q v^0_1 \otimes v^1_1)+\alpha_{010}^{111}(v^1_1\otimes q v^0_1+v^0_1\otimes v^1_1\\
&=&(\alpha_{011}^{111}+q\alpha_{010}^{111}) v^1_1\otimes v^0_1 +(\alpha_{010}^{111}-q\alpha_{011}^{111}) v^0_1\otimes v^1_1.
\eas
It follows that we can take \(\alpha_{011}^{111}=-\frac{q}{1+q^2}\) and \(\alpha_{010}^{111}=\frac{1}{1+q^2}\).
Now take \(\lim_{q\rightarrow 0}\).
Now let \bas
v^1_1\otimes v^0_1&=&\alpha_{101}^{111}(\pi^1_q v^0_1\otimes v^0_1) + \alpha_{100}^{111} \Delta(N) \pi^0_q v^0_1\otimes v^0_1\\
&=& \alpha_{101}^{111}(v^1_1 \otimes v^0_1-q v^0_1 \otimes v^1_1)
+\alpha_{100}^{111}(v^1_1\otimes q v^0_1+v^0_1\otimes v^1_1\\
&=&(\alpha_{101}^{111}
+q\alpha_{100}^{111}) v^1_1\otimes v^0_1 
+(\alpha_{100}^{111}-q\alpha_{101}^{111}) v^0_1\otimes v^1_1.
\eas
It follows that we can take \(\alpha_{101}^{111}=\frac{1}{1+q^2}\) 
and \(\alpha_{100}^{111}=\frac{q}{1+q^2}\).

We now have
\bas
\begin{pmatrix} v^1_1\otimes v^0_1\\v^0_1\otimes v^1_1\end{pmatrix}&=&\frac{1}{1+q^2}\begin{pmatrix}1&-q\\q&1 \end{pmatrix}\begin{pmatrix}
\Delta(N) \pi^0_q v^0_1\otimes v^0_1
\\ 
\pi^1_q v^0_1\otimes v^0_1
\end{pmatrix}
\eas
\fi
Let \([n]=\frac{q^n-q^{-n}}{q-q^{-1}}\),
\(v^{(i)}_m=\frac{1}{[i]_q} v^i_m\) and \(\hat{v}^{(i)}_m=\frac{1}{[i]_q} \hat{v}^i_m\).
Notice that \(\lim_{q\downarrow 0} q^{n-1}[n]=1\). It follows that \(\lim_{q\downarrow 0} q^{\binom{n}{2}} [n]!=1\) and \(\lim_{q\downarrow 0} q^{\beta(\alpha-\beta)} \binom{\alpha}{\beta}=1\).
\iffalse
Let
\[
\pi^s_q v_a\otimes v_b =\sum_{\alpha=0}^s (-1)^\alpha q^{\alpha(a-s+1)} \left( \prod_{\beta=1}^\alpha \frac{q^{2(b-s+\beta)}-1}{q^{2(a-\beta+1)}-1} \right) v^{(s-\alpha)}_a \otimes v^{(\alpha)}_b.
\]
\fi
\bas
\pi^s_q v_a\otimes v_b& =&\sum_{i+j=s} (-1)^i q^{j(b-j+1)} \frac{[a-i]![b-j]!}{[a-s]![b-s]!}  v^{(i)}_a \otimes {v}^{(j)}_b
\\& =&\sum_{i+j=s} (-1)^i q^{j(b-j+1)}  \frac{[a-i]![b-j]!}{[a-s]![j]![b-s]![i]!}  v^{i}_a \otimes {v}^{j}_b
\\& =&\sum_{i+j=s} (-1)^i q^{j(b-j+1)}  \binom{a-i}{s-i}\binom{b-j}{s-j}  v^{i}_a \otimes {v}^{j}_b.
\eas
Notice that \(\lim_{q\downarrow 0} q^{s^2-ja-ib} \binom{a-i}{s-i}\binom{b-j}{s-j} =1\).
\begin{defn}
Let \([K;n]=\frac{K q^n-K^{-1} q^{-n}}{q-q^{-1}}\). 
%\([K;a]=\frac{K q^a- K^{-1} q^{-a}} {q-q^{-1}}\)
\end{defn}
\begin{lem}
\([K;n]N=N[K;n-2]\)
\end{lem}
\begin{proof}
\bas
[K;n]N&=&\frac{K q^n-K^{-1} q^{-n}}{q-q^{-1}} N 
\\&=&N\frac{K q^{n-2}-K^{-1} q^{-n+2}}{q-q^{-1}} 
\\&=&N[K;n-2]
\eas
\end{proof}
\begin{lem}
\([M,N^k]=[k] N^{k-1}[K;1-k]
\).
		\end{lem}
\begin{proof}
For \(k=1\) the statement is \([M,N]=[1] [K;0]=\frac{K -K^{-1} }{q-q^{-1}}\), which is true by the definition of \(U_q(\mathfrak{sl}_2)\).
Then we use induction with respect to \( k\) to show that
\bas
[M,N^{k+1}]&=&MN^k N - N^{k+1} M
\\&=& N^kM N + [k] N^{k-1}[K;1-k]N - N^{k+1} M
\\&=&  N^k [K;0] + [k] N^{k}[K;-1-k] 
\\&=& \frac{N^k}{(q-q^{-1})^2} \left\{ Kq -K q^{-1} -K^{-1}q+ K^{-1}q^{-1} + (q^k-q^{-k}) (K q^{-1-k} -K^{-1} q^{k+1})\right\}
\\&=& \frac{N^k}{(q-q^{-1})^2} \left\{ Kq -K q^{-1} -K^{-1}q+ K^{-1}q^{-1} + K q^{-1} -K q^{-1-2k} - K^{-1} q^{2k+1} + K^{-1} q \right\}
\\&=& \frac{N^k}{(q-q^{-1})^2} \left\{ Kq  + K^{-1}q^{-1}  -K q^{-1-2k} - K^{-1} q^{2k+1}  \right\}
\\&=& \frac{N^k}{(q-q^{-1})^2} (q^{k+1}-q^{-k-1}) (K q^{-k} - K^{-1} q^{k} ) 
\\&=& [k+1] N^k [K;1-(k+1)] 
\eas
\end{proof}
\begin{cor}
\(M v^k_a=[k][a+1-k] v^{k-1}_a\)
\end{cor}
\begin{proof}
\(M v^k_a=[k] N^{k-1}[K;1-k] v^0_a=[k] N^{k-1} \frac{ q^{a+1-k}- q^{-a+k-1}}{q-q^{-1}}v^0_a=[k][a+1-k] v^{k-1}_a\)
\end{proof}
\iffalse
\begin{lem}
\([M,(NK)^k]=[k] (NK)^{k-1}[K;1-k] K
\).
		\end{lem}
\begin{proof}
Let \(k=1\). Then \([M,NK]=MNK-NKM=[K;0] K +NMK-NKM=[K;0] K +q^{-2} NKM-NKM\)
Let \(v_m\in\ker_M\). Then \([M,NK]v_m=MNK v_m=MN q^m v_m=[M,N] q^m v_m =[K;0] q^m v_m=[K;0]K v_m\).
Then we use induction with respect to \( k\) to show that
\bas
[M,(NK)^{k+1}]&=&M(NK)^k  NK - (NK)^{k+1} M
\\&=& (NK)^kM NK + [k](NK)^{k-1}[K;1-k]KNK  - (NK)^{k+1} M
\\&=& (NK)^k[K;0]K +(NK)^k NM K  + [k] (NK)^{k-1}KN[K;-1-k]K  - (NK)^{k+1} M
\\&=& (NK)^k[K;0]K +(NK)^k K  NM  + [k] (NK)^{k-1}KN[K;-1-k]K  - (NK)^{k+1} M
\\&=& (NK)^k[K;0]K   + [k] (NK)^{k}[K;-1-k]  K
\\&=& [k+1] (NK)^k [K;-k]K.
\eas
\end{proof}
\begin{cor}
\(M \hat{v}^k_a=[k][a+1-k]q^a \hat{v}^{k-1}_a\)
\end{cor}
\begin{proof}
\(M \hat{v}^k_a=[k] (NK)^{k-1}[K;1-k] K v^0_a=[k] (NK)^{k-1} \frac{q^{a+1-k}- q^{-a+k-1}}{q-q^{-1}}Kv^0_a=[k][a+1-k] q^a \hat{v}^{k-1}_a\)
\end{proof}
\fi
\begin{thm}
If \(v_a\otimes v_b\in \ker\Delta(M)\), then \(\pi^s_q v_a\otimes v_b\in \ker\Delta(M)\) and \(\Delta(K)\pi^s_q v_a\otimes v_b=q^{a+b-2s} \pi^s_q v_a\otimes v_b\).
\end{thm}
\begin{proof}
\bas
\Delta(M) \pi^s_q v_a\otimes v_b&=& \sum_{i+j=s} (-1)^i q^{j(b-j+1)} \binom{a-i}{s-i}\binom{b-j}{s-j}  M  v^{i}_a \otimes K {v}^{j}_b\\&&
+\sum_{i+j=s} (-1)^i q^{j(b-j+1)} \binom{a-i}{s-i}\binom{b-j}{s-j}  v^{i}_a \otimes M {v}^{j}_b
\\&=& \sum_{i+j=s} (-1)^i q^{j(b-j+1)} \frac{[a-i]![b-j]!}{[a-s]![b-s]![j]![i]!} [i][a+1-i]  v^{i-1}_a \otimes q^{b-2j} {v}^{j}_b\\&&
+\sum_{i+j=s} (-1)^i q^{j(b-j+1)} \frac{[a-i]![b-j]!}{[a-s]![b-s]![i]![j]!}   v^{i}_a \otimes  [j][b+1-j] {v}^{j-1}_b
\\&=& \sum_{i+j=s} (-1)^i q^{(j+1)(b-j)} \frac{[a-i+1]![b-j]!}{[a-s]![b-s]![j]![i-1]!}   v^{i-1}_a \otimes {v}^{j}_b\\&&
+\sum_{i+j=s} (-1)^i q^{j(b-j+1)} \frac{[a-i]![b+1-j]!}{[a-s]![b-s]![i]![j-1]!}   v^{i}_a \otimes  {v}^{j-1}_b
\\&=&-\sum_{i+j=s-1} (-1)^i q^{(j+1)(b-j)} \frac{[a-i]![b-j]!}{[a-s]![b-s]![j]![i]!}   v^{i}_a \otimes {v}^{j}_b\\&&
+\sum_{i+j=s-1} (-1)^i q^{(j+1)(b-j)} \frac{[a-i]![b-j]!}{[a-s]![b-s]![i]![j]!}   v^{i}_a \otimes  {v}^{j}_b
\\&=&0,
\eas
and
\bas
\Delta(K) \pi^s_q v_a\otimes v_b&=& 
\sum_{i+j=s} (-1)^i q^{j(b-j+1)}  \binom{a-i}{s-i}\binom{b-j}{s-j} K  v^{i}_a \otimes K {v}^{j}_b
\\&=&\sum_{i+j=s} (-1)^i q^{j(b-j+1)}  \binom{a-i}{s-i}\binom{b-j}{s-j} q^{a-2i}  v^{i}_a \otimes q^{b-2j} {v}^{j}_b
\\&=& q^{a+b-2s} \pi^s_q v_a\otimes v_b.
\eas
\end{proof}
Let us check whether this is compatible with the earlier definitions.
Take \(a=b=1\).
\bas
\pi^1_q v_1\otimes v_1& =& \sum_{i+j=1} (-1)^i q^{j(1-j+1)}  \binom{1-i}{1-i}\binom{1-j}{1-j}  v^{i}_1 \otimes {v}^{j}_1
\\&=& q  v^{0}_1 \otimes {v}^{1}_1
-   v^{1}_1 \otimes {v}^{0}_1
\\
\Delta(N)\pi^0_q v_1\otimes v_1& =& N v_1^0 \otimes v_1^0 +K^{-1} v_1^0 \otimes N v_1^0
\\&=&
 v_1^1 \otimes v_1^0 +q^{-1} v_1^0 \otimes  v_1^1
\eas
Thus
\bas
\begin{pmatrix} \Delta(N)\pi^0_q v_1\otimes v_1\\ \pi^1_q v_1\otimes v_1\end{pmatrix} =
\begin{pmatrix} 1 & q^{-1}\\ -1&q \end{pmatrix}\begin{pmatrix} v^{1}_1 \otimes {v}^{0}_1 \\ v^{0}_1 \otimes {v}^{1}_1\end{pmatrix}
\eas
and
\bas
\begin{pmatrix} v^{1}_1 \otimes {v}^{0}_1 \\ v^{0}_1 \otimes {v}^{1}_1\end{pmatrix}&=&\frac{1}{q+q^{-1}}\begin{pmatrix} q & -q^{-1}\\ 1&1 \end{pmatrix}\begin{pmatrix} \Delta(N)\pi^0_q v_1\otimes v_1\\ \pi^1_q v_1\otimes v_1\end{pmatrix}
\\&=&\frac{1}{q^2+1}\begin{pmatrix} q^2 & -1\\ q&q \end{pmatrix}\begin{pmatrix} \Delta(N)\pi^0_q v_1\otimes v_1\\ \pi^1_q v_1\otimes v_1\end{pmatrix}
\eas
Then
\[
\lim_{q\downarrow 0}\begin{pmatrix} v^{1}_1 \otimes {v}^{0}_1 \\ v^{0}_1 \otimes {v}^{1}_1\end{pmatrix}
=\begin{pmatrix} 0 & -1\\ 0&0 \end{pmatrix}\begin{pmatrix} \Delta(N)\pi^0_0 v_1\otimes v_1\\ \pi^1_0 v_1\otimes v_1\end{pmatrix}
=\begin{pmatrix}-  \pi^1_0 v_1\otimes v_1\\0\end{pmatrix}\]
\iffalse
\bas
\pi^1_q v_a\otimes v_b& =&
\sum_{\alpha=0}^1 (-1)^\alpha q^{(1-\alpha)(\alpha+1)} \left( \prod_{\beta=1}^\alpha \frac{q^{2(b-1+\beta)}-1}{q^{2(a-\beta+1}-1} \right) v^{(\alpha)}_a \otimes v^{(1-\alpha)}_b\\
&=&
q v^{(0)}_a \otimes v^{(1)}_b-
\left(  \frac{q^{2b}-1}{q^{2a}-1} \right) v^{(1)}_a \otimes v^{(0)}_b\\
\eas
\fi
Let \(r=i+j=k+p\). Then
\bas
{(r)!}^4 {{m}\choose{r}}{{n}\choose{r}} {{m+n-r+1}\choose{r}}
\eas
\fi
\iffalse
\section{Kassel}
In this section we follow Kassel in the definition of transvectant and $3j$-symbols.
\begin{lem}
Let \(v^{(n)}\) be a highest weight vector of weight \(n\) in \(V_n\)
and \(v^{(m)}\) be a highest weight vector of weight \(m\) in \(V_m\).
Let is define \(v_p^{(n)}=\frac{1}{p!} F^p v^{(n)}\) and \(v_p^{(m)}=\frac{1}{p!} F^p v^{(m)}\) for all \(p \geq 0\).
Then
\bas
v^{(n+m-2p)}=\sum_{i=0}^p (-1)^i \frac{(m-p+i)!(n-i)!}{(m-p)!n!} v_i^{(n)} \otimes v_{p-i}^{(m)}
\eas
is a highest weight vector of weight \(n+m-2p\) in \(V_n\otimes V_m\).
\end{lem}
We wish to go one step further
and address the following problem. We now have two bases of \(V_n\otimes V_m\) at
our disposal. They are of different natures: the first one, adapted to the
tensor product, is the set
\bas
\{ v_i^{(n)}\otimes v_j^{(m)} \}_{i=0,\cdots,n, j=0,\dots, m};
\eas
the second one, formed by the vectors
\bas
v_k^{(n+m-2p)} =\frac{1}{k!} F^k v^{(n+m-2p)}
\eas
with \(0 \leq p \leq m \) and \(0 \leq k \leq n + m - 2p\), is better adapted to the \(U\) -
module structure. Comparing both bases leads us to the so-called 
Clebsch-Gordan coefficients
\bas
\begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix}
\eas
defined for \(0 \leq p \leq m \) and \(0 \leq k \leq n + m - 2p\) by
\bas
v_k^{(n+m-2p)} =\sum_{i=0,\cdots,n,j=0,\cdots m} \begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix} v_i^{(n)} \otimes v_{j}^{(m)}
\eas
The remainder of this section is devoted to a few properties of these coefficients, also called \(3j\)-symbols in the physics literature.
\begin{lem}
Fix \(p\) and \(k\). The vector \( v_k^{(n+m-2p)}\) is a linear combination of vectors of the form \(v_i^{(n)}\otimes v_{p-i+k}^{(m)}\).
Therefore, we have
\bas
\begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix}=0
\eas
if \(i+j\neq p+k\).
We also have the induction relation
\bas
\begin{pmatrix} n&m&n+m-2p\\i&j+1&k+1\end{pmatrix}=\frac{j+1+i}{k+1}
\begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix}.
\eas
\end{lem}
\begin{proof}
\bas
v_{k+1}^{(n+m-2p)}&=&\frac{1}{k+1} F v_k^{(n+m-2p)} \\
 &=&
\frac{1}{k+1} \sum_{i=0,\cdots,n,j=0,\cdots m} \begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix} (i+1) v_{i+1}^{(n)} \otimes v_{j}^{(m)}
\\&+&\frac{1}{k+1} \sum_{i=0,\cdots,n,j=0,\cdots m} \begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix} (j+1) v_i^{(n)} \otimes v_{j+1}^{(m)}
 \\&=&
\frac{1}{k+1} \sum_{i=0,\cdots,n,j=0,\cdots m} \begin{pmatrix} n&m&n+m-2p\\i-1&j+1&k\end{pmatrix} i v_{i}^{(n)} \otimes v_{j+1}^{(m)}
\\&+&\frac{1}{k+1} \sum_{i=0,\cdots,n,j=0,\cdots m} \begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix} (j+1) v_i^{(n)} \otimes v_{j+1}^{(m)}
\eas
It is not clear why the result follows.
\end{proof}
Let us now compute the \(3j\)-symbols in the simplest nontrivial case \(i+j=p+k=1\).
\bas
v_1^{(n+m)} &=&\sum_{i+j=1} \begin{pmatrix} n&m&n+m\\i&j&1\end{pmatrix} v_i^{(n)} \otimes v_{j}^{(m)}\\
\\&=&\begin{pmatrix} n&m&n+m\\0&1&1\end{pmatrix} v_0^{(n)} \otimes v_{1}^{(m)}+\begin{pmatrix} n&m&n+m\\1&0&1\end{pmatrix} v_1^{(n)} \otimes v_{0}^{(m)}\\
v_0^{(n+m-2)} &=&\sum_{i+j=1} \begin{pmatrix} n&m&n+m-2\\i&j&0\end{pmatrix} v_i^{(n)} \otimes v_{j}^{(m)}\\
&=&  \begin{pmatrix} n&m&n+m-2\\0&1&0\end{pmatrix} v_0^{(n)} \otimes v_{1}^{(m)}+ \begin{pmatrix} n&m&n+m-2\\1&0&0\end{pmatrix} v_1^{(n)} \otimes v_{0}^{(m)}
\eas
On the other hand we have
\bas
v_1^{(n+m)} &=&\Delta(F) v^{(n+m)}=\Delta(F) v_0^{(n)}\otimes v_0^{(m)}=v_0^{(n)} \otimes v_{1}^{(m)}+v_1^{(n)} \otimes v_{0}^{(m)}\\
v_0^{(n+m-2)} &=&
\sum_{i=0}^1 (-1)^i \frac{(m-p+i)!(n-i)!}{(m-p)!n!} v_i^{(n)} \otimes v_{p-i}^{(m)}= v_0^{(n)} \otimes v_{1}^{(m)}
- \frac{m}{n} v_1^{(n)} \otimes v_{0}^{(m)}
\eas
In other words
\ba\label{EQU}
\begin{pmatrix} v_1^{(n+m)} \\ v_0^{(n+m-2)}\end{pmatrix}
&=&\begin{pmatrix} 1& 1\\1 &-\frac{m}{n} \end{pmatrix} \begin{pmatrix} v_0^{(n)} \otimes v_{1}^{(m)}\\v_1^{(n)} \otimes v_{0}^{(m)}\end{pmatrix}
\ea
It is difficult to see an orthogonal matrix here,
but if we compute the transpose induced by the inner product such that \((Fv,w)=(v,Ew)\), in other words \(F^t=E\), then we obtain
\bas
A&=&\begin{pmatrix} 1& 1\\1 &-\frac{m}{n} \end{pmatrix} ,\quad A^t=\begin{pmatrix} \frac{m}{m+n}& m\\\frac{n}{n+m} &-m \end{pmatrix} \eas
and we
see that
\bas
A A^t=\begin{pmatrix} 1& 0\\0 &m(m+n) \end{pmatrix} \eas
That this is not the identity is caused by the fact that we use an orthogonal, but not orthonormal system.
The recipe is: multiply the first column with \(\| v_0^{(n)} \otimes v_{1}^{(m)}\|^2=\binom{m}{1}\binom{n}{0}=m\),
the second column with \(\| v_1^{(n)} \otimes v_{0}^{(m)}\|^2=\binom{m}{0}\binom{n}{1}=n\), and divide the first row by 
\(\|v_1^{(n+m)}\|^2=\binom{m+n}{1}=m+n\) and the second row by \(\|v_0^{(n+m-2)}\|^2=\binom{n+m-2}{0}=1\).
Then take the usual transpose.

It follows from \cite[Proposition VII.7.5]{kassel2012quantum} that 
\bas
v_i^{(n)}\otimes v_j^{(m)}&=&
\binom{n}{i}\binom{m}{j} 
\sum_{p+k=i+j} \frac{\begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix}}{\binom{n+m-2p}{k}}
v_k^{(n+m-2p)}
\eas
In particular,
\bas
v_0^{(n)}\otimes v_1^{(m)}&=&
\frac{m}{n+m}
\begin{pmatrix} n&m&n+m\\0&1&1\end{pmatrix}
v_1^{(n+m)}
+
m
\begin{pmatrix} n&m&n+m-2\\0&1&0\end{pmatrix}
v_0^{(n+m-2)}
\\&=&
\frac{m}{n+m}
v_1^{(n+m)}
+
m
v_0^{(n+m-2)}\\
v_1^{(n)}\otimes v_0^{(m)}&=&
\frac{n}{n+m} \begin{pmatrix} n&m&n+m\\1&0&1\end{pmatrix} v_1^{(n+m)}
+n \begin{pmatrix} n&m&n+m-2\\1&0&0\end{pmatrix} v_0^{(n+m-2)}
\\&=&
\frac{n}{n+m}  v_1^{(n+m)}
-m v_0^{(n+m-2)}
\eas
In other words
\bas
\begin{pmatrix} v_0^{(n)}\otimes v_1^{(m)}\\v_1^{(n)}\otimes v_0^{(m)}\end{pmatrix}
&=&\begin{pmatrix}\frac{m}{n+m} &m \\ \frac{n}{n+m} & -m\end{pmatrix}\begin{pmatrix} v_1^{(n+m)} \\ v_0^{(n+m-2)}\end{pmatrix}
\eas
This is a contradiction with Equation (\ref{EQU}), since it is supposed to be the inverse.

We now turn to the orthogonality statements in \cite[Proposition VII.7.5]{kassel2012quantum}.
The first statement is that
\bas
0&=&\sum_{i,j} \binom{n}{i}\binom{m}{j} \begin{pmatrix} n&m&n+m-2p\\i&j&k\end{pmatrix} \begin{pmatrix} n&m&n+m-2q\\i&j&l\end{pmatrix}
\eas
when \(p\neq q\) or \(k\neq l\).
Let us take \(p=0, k=1, q=1, l=0\).
Then we find
\bas
0&=&\sum_{i+j=1} \binom{n}{i}\binom{m}{j} \begin{pmatrix} n&m&n+m\\i&j&1\end{pmatrix} \begin{pmatrix} n&m&n+m-2\\i&j&0\end{pmatrix}
\\&=&
m \begin{pmatrix} n&m&n+m\\0&1&1\end{pmatrix} \begin{pmatrix} n&m&n+m-2\\0&1&0\end{pmatrix}
+ n \begin{pmatrix} n&m&n+m\\1&0&1\end{pmatrix} \begin{pmatrix} n&m&n+m-2\\1&0&0\end{pmatrix}
\\&=&
m  
+ n (-\frac{m}{n})
\\&=&0.
\eas
My conclusion: orthogonality holds, but the formula in (c) is wrong.
Let us take \(p=0, k=1\).
\bas
0&=&\sum_{i+j=1} \binom{n}{i}\binom{m}{j} \begin{pmatrix} n&m&n+m\\i&j&1\end{pmatrix}^2 
\\&=&
m \begin{pmatrix} n&m&n+m\\0&1&1\end{pmatrix}^2 
+ n \begin{pmatrix} n&m&n+m\\1&0&1\end{pmatrix}^2 
\\&=&m+n
\\&=&\binom{n+m-2p}{k}
\eas
Let us take \(p=0, k=1\).
\bas
0&=&\sum_{i+j=1} \binom{n}{i}\binom{m}{j} \begin{pmatrix} n&m&n+m-2\\i&j&0\end{pmatrix}^2 
\\&=&
m \begin{pmatrix} n&m&n+m-2\\0&1&0\end{pmatrix}^2 
+ n \begin{pmatrix} n&m&n+m-2\\1&0&0\end{pmatrix}^2 
\\&=&m+n\frac{m^2}{n^2}
\\&=&\frac{m(m+n)}{n}
\eas
This implies (b) is wrong. And therefore (c) is wrong. Question: what is the right formula?
\fi
\iffalse
\subsection{Letter to Kassel}
Dear Professor Kassel,

we came in contact with the problem of inverting the Clebsch-Gordan expressions,
that is, expressing the two-tensors in tems of \(F\)-orbits of transvectants,
in our research into the unique normal form of vector fields with in three dimensions with an irreducible linear term.

After obtaining an inverse procedure based on Gauss-elimination,
we came on the method described in your Quantum Groups book in Proposition VII.7.5.

Since having a method based on orthogonality has an obvious advantage when it comes to inversion,
we have tried to implement your method in the classical case \(q=1\).
We, however, found that it is not working correctly as stated.
We will illustrate this in the simplest nontrivial case.

We take \(i+j=p+k=1\).
Then
\bas
v^{n+m-2}&=&v^{(n)} \otimes v_1^{(m)}-\frac{m}{n} v_1^{(n)}\otimes v^{(m)},\\
v_1^{n+m}&=&v^{(n)} \otimes v_1^{(m)}+v_1^{(n)}\otimes v^{(m)}.
\eas
According to Proposition VII.7.5 (c), the inverse expression should be
\bas
v^{(n)}\otimes v_1^{(m)}&=&
\frac{m}{n+m}
\begin{pmatrix} n&m&n+m\\0&1&1\end{pmatrix}
v_1^{(n+m)}
+
m
\begin{pmatrix} n&m&n+m-2\\0&1&0\end{pmatrix}
v^{(n+m-2)}
\\&=&
\frac{m}{n+m}
v_1^{(n+m)}
+
m
v^{(n+m-2)}\\
v_1^{(n)}\otimes v^{(m)}&=&
\frac{n}{n+m} \begin{pmatrix} n&m&n+m\\1&0&1\end{pmatrix} v_1^{(n+m)}
+n \begin{pmatrix} n&m&n+m-2\\1&0&0\end{pmatrix} v^{(n+m-2)}
\\&=&
\frac{n}{n+m}  v_1^{(n+m)}
-m v^{(n+m-2)}
\eas
The two sets of equations are clearly incompatible, since all terms in the previous equations should have \(m+n\) in the denominator.
We checked this is not in the AMS Errata list of your book.
Nevertheless we convinced ourselves that the method works in the sense that the matrices involved are orthogonal (but not orthonormal), using the given inner product.
It is not difficult to find the correction terms.

So our question is
\begin{itemize}
\item
Is there a (classical) source for this method which ideally gives a correct formulation?
\item
If so, is there a proof available?
\end{itemize}
%Since a large body of the literature assumes orthonormality this does not seem to be a problem.
We hope that you can help us out on this issue.
\newline
Sincerely yours,
\newline
Fahimeh Mokhtari and Jan A. Sanders
\newline
Free University Amsterdam (VU)
\newline
Faculty of Science
\newline
Department of Mathematics.
\fi
\iffalse
\subsection{Duality and traces (after Kassel)}
WARNING: copy-paste of Kassel, do not use this text as is.

All vector spaces considered in this section are assumed to be finite-dimensional. If \(V\) is such a vector space, we denote a basis of \(V\) by \(\{v_i\}_i\) using
the corresponding lower-case letter for vectors. The (standard) dual basis in the dual
vector space \(V^\star\) is denoted \(\{v^i\}_i\). Using these bases, the evaluation map
can be redefined by
\[
v^j(v_i)=\mathrm{ev}_V(v_i\otimes v^j)=\langle v_i,v^j\rangle=\delta_{i}^{j}.
\]
Alternatively, if we have an inner product \((\cdot,\cdot)_V\) on \(V\), we define a dual basis \(\bar{v}^i\) by
\[
\bar{v}^j(v_i)=\mathrm{in}_V(v_i\otimes \bar{v}^j)=( v_i,{v}_j)_V.
\]
\begin{rem}
In \cite{frenkel2010categorifying} the dual basis is defined as
\[
\hat{v}_n^i=\frac{1}{\binom{n}{i}} v_i^n,
\]
in the case that \(V\) is an \(n+1\)-dimensionaL irreducible \(\Sl\)-representation, which seems to be the way Kassel does it too.
\end{rem}
If the basis \(\{v_i\}_i\) is orthogonal, then \(\bar{v}^j(v_i)=(v_j,{v}_j)_V v^j(v_i)\), that is \(\bar{v}^j= (v_j,{v}_j)_V v^j\).
Let us express the isomorphism \(\lambda_{U,V} : V \otimes U^\star \cong \mathrm{Hom}(U, V)\) of \cite[Corollary 2.3]{kassel2012quantum}
in terms of bases. Let \(f : U \rightarrow V\) be a linear map. Using bases for \(U\)
and \(V\), we have
\ba\label{eq:comp}
f(u_j)=\sum_i f_j^i v_i
\ea
for some family \(\{f^i_j\}_{ij}\) of scalars. It is easily checked that
\[
f=\lambda_{U,V}(\sum_{ij}f^i_j v_i \otimes u^j)=(?)\lambda_{U,V}(\sum_{ij}\bar{f}^i_j v_i \otimes \bar{u}^j).
\]
In particular, taking for \(f\) the identity of \(V\), we get
\[
\mathrm{id}_V=\lambda_{V,V}(\sum_{i} v_i \otimes v^i).
\]
This allows us to define the coevaluation map of any finite-dimensional
vector space \(V\) as the linear maps \(\delta_V, \bar{\delta}_V : k \rightarrow V \otimes V^\star\) defined by
\bas
\delta_V(1)&=&\lambda_{V,V}^{-1}(\mathrm{id}_V)=\sum_{i} v_i \otimes v^i,\\
\bar{\delta}_V(1)&=(?)&\lambda_{V,V}^{-1}(\mathrm{id}_V)=\sum_{i} v_i \otimes \bar{v}^i.
\eas
By its very definition, the map \(\delta_V\) is independent of the choice of a basis. We
now record some relations between the evaluation and coevaluation maps.
These relations will turn out to be fundamental when we define duality in
categories in \cite[Chapter XIV]{kassel2012quantum}.
\begin{prop}. The composition of the maps
\[
V\stackrel{\delta_V\otimes \mathrm{id}_V}{\longrightarrow}V\otimes V^\star\otimes V\stackrel{\mathrm{id}_V\otimes \mathrm{ev}_{V}}{\longrightarrow} V
\]
is equal to the identity of V. Similarly, the composition of the maps
\[
V^\star\stackrel{\mathrm{id}_{V^\star}\otimes \delta_V}{\longrightarrow}V^\star\otimes V \otimes V^\star\stackrel{\mathrm{in}_V\otimes \mathrm{id}_{V^\star}}{\longrightarrow} V^\star
\]
is equal to the identity of \(V^\star\).
\end{prop}
\begin{proof}
Let \(\alpha^i=v^i(v)\in k\). Then \(v=\sum_i \alpha^i v_i\).
\bas
\mathrm{id}_V\otimes \mathrm{ev}_{V}(\delta_V\otimes id_V (1\otimes v))&=&\mathrm{id}_V\otimes \mathrm{ev}_{V}(\delta_V(1)\otimes v)\\&=&
\mathrm{id}_V\otimes \mathrm{ev}_{V}(\sum_i v_i\otimes v^i \otimes v)
=\sum_i v_i \alpha^i=v
\eas
%Immediate.
\end{proof}
Let us recall the operation of transposition. For a linear map \(f : U \rightarrow V\),
define its {\em transpose} \(f^\star : V^\star \rightarrow U^\star \) as the linear map defined for all \(\alpha\in V^\star\)
and all \(u \in U\) by
\[
\langle f^\star(\alpha),u\rangle= \langle\alpha,f(u)\rangle,
\]
or
\[
( f^\perp(\alpha),u)_U= ( \bar{\alpha},f(u))_V .
\]
In other words,
\(f^\star\) and \(f^\perp\)
are the unique linear map such that the squares
\[ \psset{arrows=->, arrowinset=0.25, linewidth=0.6pt, nodesep=3pt, labelsep=2pt, rowsep=0.7cm, colsep = 1.1cm, shortput =tablr}
 \everypsbox{\scriptstyle}
 \]
\[ \begin{tikzcd}
V^\star\otimes U \arrow{r}{f^\star \otimes \mathrm{id}_U} \arrow[swap]{d}{\mathrm{id}_{V^\star}\otimes f} & U^\star\otimes U \arrow{d}{\mathrm{ev}_U} \\%
V^\star\otimes V \arrow{r}{\mathrm{ev}_V}& k
\end{tikzcd}
\]
\[ \begin{tikzcd}
V^\star\otimes U \arrow{r}{f^\perp \otimes \mathrm{id}_U} \arrow[swap]{d}{\mathrm{id}_{V^\star}\otimes f} & U^\star\otimes U \arrow{d}{\mathrm{in}_U} \\%
V^\star\otimes V \arrow{r}{\mathrm{in}_V}& k
\end{tikzcd}
\]
commutes. The transposition may be recovered from the evaluation and
coevaluation maps as shown in the following result whose proof is left to
the reader.
\begin{prop} Let \(f : U \rightarrow V\) be a linear map. Then the transpose
\(f^\star\) is equal to the composition of the maps
\bas
V^\star\stackrel{\mathrm{id}_{V^\star}\otimes \delta_U}{\longrightarrow}V^\star\otimes U\otimes U^\star \stackrel{\mathrm{id}_{V^\star}\otimes f\otimes \mathrm{id}_{U^\star}}{\longrightarrow} V^\star\otimes V\otimes U^\star\stackrel{\mathrm{ev}_V\otimes \mathrm{id}_{U^\star}}{\longrightarrow}U^\star.
\\
v^j\stackrel{\mathrm{id}_{V^\star}\otimes \delta_U}{\longrightarrow}\sum_i v^j\otimes u_i\otimes u^i \stackrel{\mathrm{id}_{V^\star}\otimes f\otimes \mathrm{id}_{U^\star}}{\longrightarrow}\sum_i  v^j\otimes f(u_i)\otimes u^j\stackrel{\mathrm{ev}_V\otimes \mathrm{id}_{U^\star}}{\longrightarrow}\sum_i f_j^i u^j,
\eas
where \(f_j^i=\langle f(u_i) , v^j\rangle \) and \(f^\perp\) is equal to the composition of the maps (???)
\bas
V^\star\stackrel{\mathrm{id}_{V^\star}\otimes \bar{\delta}_U}{\longrightarrow}V^\star\otimes U\otimes U^\star \stackrel{\mathrm{id}_{V^\star}\otimes f\otimes \mathrm{id}_{U^\star}}{\longrightarrow} V^\star\otimes V\otimes U^\star\stackrel{\mathrm{in}_V\otimes \mathrm{id}_{U^\star}}{\longrightarrow}U^\star,\\
\bar{v}^j\stackrel{\mathrm{id}_{V^\star}\otimes \bar{\delta}_U}{\longrightarrow}\sum_i \bar{v}^j\otimes u_i\otimes \bar{u}^i \stackrel{\mathrm{id}_{V^\star}\otimes f\otimes \mathrm{id}_{U^\star}}{\longrightarrow} \sum_i \bar{v}^j\otimes f(u_i)\otimes \bar{u}^i\stackrel{\mathrm{in}_V\otimes \mathrm{id}_{U^\star}}{\longrightarrow}\sum_i (v_j\otimes f(u_i))_V \otimes \bar{u}^i.
\eas
\end{prop}
Observe that if (\ref{eq:comp}) holds, then
\ba
f^\star(v^j)=\sum_i f_i^j u^i,\quad f^\perp(\bar{v}^j)=\sum_i (v_j, f(u_i))_V \bar{u}^i
=\sum_i \bar{f}_i^j \bar{u}^i
\ea
We thus see that transposition amounts to exchanging upper and lower
indices.
Since \( \bar{u}^i=(u_i,u_i)_U u^i\), we find that \[\bar{f}_i^j=(v_j, f(u_i))_V (u_i,u_i)_U=(v_j,\sum_k f_i^k v_k  )_V (u_i,u_i)_U=(v_j, v_j  )_V (u_i,u_i)_U f_i^j.\]
\fi
\section{Clebsch-Gordan symbols, a rational approach}
The following is based on \cite[Chapter XIV]{kassel2012quantum}.
There an explicit method is given to express elements in \(V_m\otimes V_n\) in terms of the \(N\)-orbits of their transvectants (these are given in Lemma VII.7.2, loc. cit.).
The only problem with this formula is that it implicitly assumes the norm of the transvectant to be \(1\).
Here we present a corrected version of this, restricted to the classical case \(q=1\), the quantum case should be completely similar.
The rational approach that is followed, see also \cite{rationalCGC2018}, does avoid the square roots that appear in the usual quantum mechanical approach,
where one works with an orthonormal base; we are happy with orthogonality.
It may also be useful in the categorification program, see \cite{frenkel2010categorifying}

Let \(V\) be an \(\Sl\)-module.
We assume \(\ker M|V\) to be a direct sum of finite-dimensional \(H\)-eigenspaces \(V_m\).
We choose a basis for \(\ker M\) consisting of eigenvectors, say \[\langle v_{\{1\}}^{m_1},\ldots,v_{\{k_{m_1}\}}^{m_1},\ldots,v_{\{1\}}^{m_k},\ldots,v_{\{k_{m_k}\}}^{m_k}\rangle.\]
Then we construct the standard dual basis \(\langle v^{\{1\}}_{m_1},\ldots,v^{\{k_{m_1}\}}_{m_1},\ldots,v^{\{1\}}_{m_k},\ldots,v^{\{k_{m_k}\}}_{m_k}\rangle\)
and define the standard inner product \(( v_{\{i\}}^k, v_{\{j\}}^l)_{\ker M}=v^{\{i\}}_k(v_{\{j\}}^l)=\delta_{i,j}\delta_{k,l}\), with linear extension defined on all of \(\ker M\).
Then we let for given \(v^m \in\ker M \) with \(H\)-eigenvalue \(m\),
\bas
v_i^m= N^i v^m, \quad v^m\in\ker M, \quad v_i^{(m)}=\frac{1}{i!} v_i^m, N v_i^{(m)}=\frac{1}{i!} N v_i^m=(i+1) v_{i+1}^{(m)}. 
\eas
%\quad v_i^{(m)}=\frac{1}{i!} N^i v^m, i=0,\ldots,m
We denote the space spanned by \(v_i^m, i=0,\ldots,m\) by \(V_m\).
We then define an induced inner product on \( V\) by definining it on eigenvectors by 
\[ (v_i^{(m)},w_j^{(n)})_V=\binom{m}{i}\delta_{i,j}\delta_{m,n}(v^m,w^n)_{\ker M},\quad v^m,w^n\in\ker M\]
and then by linear extension on all of \(V\). The \(\delta_{m,n}\) is not really necessary here, it follows from the definition of \((\cdot,\cdot)_{\ker M}\).
%Furthermore, we let \(v^{\langle m\rangle}_i=\frac{1}{\sqrt{\binom{m}{i}}} v^{(m)}_i\), with \(\|v^{\langle m\rangle}_i\|^2=1\).
%\begin{rem}
%Check this notation is used at all.
%\end{rem}
\iffalse
\begin{rem}
If we let \(v^m=x^m\), \(N=y\frac{\partial}{\partial x}\) and \(N=x\frac{\partial}{\partial y}\), then \(N^i v^m= \frac{m!}{(m-i)!} x^{m-i} y^i=i! \binom{m}{i} x^{m-i} y^i\).
We define \(v^m_i=\frac{m!}{(m-i)!} x^{m-i} y^i\) and \(v^{(m)}_i=\binom{m}{i} x^{m-i} y^i=\frac{1}{i!} v^m_i\). 
\end{rem}
\fi
\iffalse
\begin{rem}
The groundform for \(V_m\) is in symbolic notation (cf \cite{olver1999classical}) \(G_v^m=(vx)^m=(v_1 x_1+v_2 x_2)^m\).
We identify  \(\binom{m}{j} v_1^{m-j}v_2^j\) with \(v_j^{(m)}\) and we write this as \(\binom{m}{j} v_1^{m-j}v_2^j\rightrightarrows v_j^{(m)}\).
It follows that \(G_v^m\rightrightarrows \sum_{j=0}^m x_1^j x_2^{m-j} v_j^{(m)}\).
% and \(v_j^{(m)}\leftleftarrows \binom{m}{j} v_1^{m-j}v_2^j\).
If we let \(\hat{N}=v_2\frac{\partial}{\partial v_1}\) and \(\hat{M}=v_1\frac{\partial}{\partial v_2}\), then \(\hat{N}^i v_1^{m}= \frac{m!}{(m-i)!}v_1^{m-i}v_2^i =i! \binom{m}{i} v_1^{m-i} v_2^i\rightrightarrows i! v_i^{(m)}=v_i^m=N^i v^m\).
%The notation \(v_1^m\) has different meanings, depending on which side of the \(\rightrightarrows\) it appears.
\iffalse
The inner product \((v_i^{(m)},v_j^{(n)})=\delta_{i,j} \binom{m}{i}(v^m,w^n)_{\ker M}\) corresponds to the following inner product for the symbolic expressions:
\bas
(v_1^{m-j}v_2^j,v_1^{m-i}v_2^i)&\rightrightarrows&\frac{1}{\binom{m}{i}\binom{m}{j}} (v_j^{(m)},v_i^{(m)})
= \delta_{i,j} \frac{1}{\binom{m}{i}}(v^m,v^m)_{\ker M}.
\eas
\fi
\end{rem}
\fi
\begin{lem} 
One has \(N^\perp=M\) and \(M^\perp=N\), where \(N^\perp\) is the transpose of \(N\) with respect to the inner product \((\cdot,\cdot)_V\):
\[
( N v , w )_V =(v, Mw)_V, \quad v,w\in V
\]
\end{lem}
\begin{proof}
We compute the two sides on basis vectors:
\bas
(N v_i^{(m)},w_j^{(n)})_V&=& ( (i+1) v_{i+1}^{(m)},w_j^{(n)})_V=(i+1)\binom{m}{i+1}\delta_{i+1,j}\delta_{m,n}(v^m,w^n)_{\ker M}
\\&=&(m-i)\binom{m}{i}\delta_{i+1,j}\delta_{m,n}(v^m,w^n)_{\ker M},\\
		   (v_i^{(m)}, M w_j^{(n)})_V&=& (v_i^{m}, \frac{1}{j!}M N^j w^{n})=(v_i^{(m)},\frac{1}{(j-1)!} (m-j+1) N^{j-1} w^{n})_V=(m-j+1) (v_i^{(m)}, w_{j-1}^{(n)})_V
\\&=& (m-i)  \binom{m}{i} \delta_{i,j-1}\delta_{m,n} (v^m,w^n)_{\ker M}
\eas
By linear extension this holds true on \(V\).
\end{proof}
\begin{rem}
Using this property, one can easily show orthogonality of the vectors \(v_i^m\) and \(v_j^n\), consistent with the \(\delta_{i,j}\) in the definition
of the inner product. 
%This is a bit of a chicken and egg question. In any case, by choosing a different factor than \( \binom{m}{i}\) one can easily loose orthogonality,
%thus making the whole setup inconsistent. It would be good to set this up a bit tighter. The proof in \cite{kassel2012quantum} did not make things any clearer to us.
\end{rem}
\iffalse
We see that \bas
\hat{N}G_m&=&x_1\frac{\partial}{\partial x_2}(v_1 x_1+v_2 x_2)^m=m x_1 v_2(v_1x_1+v_2x_2)^{m-1}
\\&=&m\sum_{i=0}^{m-1} \binom{m-1}{i} v_1^{m-1-i}v_2^{i+1} x_1^{m-i} x_2^{i}\rightrightarrows m\sum_{i=0}^{m-1}\frac{ \binom{m-1}{i}}{\binom{m}{i+1}} v_{i+1}^{(m)} \otimes  x_1^{m-i} x_2^{i}
\\&=&\sum_{i=0}^{m-1}(i+1) v_{i+1}^{(m)}  x_1^{m-i} x_2^{i}=\sum_{i=0}^{m-1}N v_{i}^{(m)}  x_1^{m-i} x_2^{i}=N\sum_{i=0}^{m-1} v_{i}^{(m)}\otimes   x_1^{m-i} x_2^{i},\\
\hat{M}G_m&=&x_2\frac{\partial}{\partial x_1}(v_1 x_1+v_2 x_2)^m=m x_2 v_1(v_1x_1+v_2x_2)^{m-1}
\\&=&m\sum_{i=0}^{m-1} \binom{m-1}{i} v_1^{m-i}v_2^{i} x_1^{m-1-i} x_2^{i+1}=\sum_{i=1}^{m} \binom{m-1}{i-1} v_1^{m+1-i}v_2^{i-1}\otimes  x_1^{m-i} x_2^{i}\\
&\rightrightarrows&m\sum_{i=0}^{m-1}\frac{ \binom{m-1}{i-1}}{\binom{m}{i-1}} v_{i-1}^{(m)} \otimes  x_1^{m-i} x_2^{i}
=\sum_{i=0}^{m-1}(m-i+1) v_{i-1}^{(m)}  x_1^{m-i} x_2^{i}\\&=&\sum_{i=0}^{m-1}M v_{i}^{(m)}  x_1^{m-i} x_2^{i}=M\sum_{i=0}^{m-1} v_{i}^{(m)} \otimes  x_1^{m-i} x_2^{i},
\eas
that is to say, the action of \(N\) is induced by the action of \(\hat{N}\), and we have \(\hat{N}G_m\rightrightarrows NG_m\), and likewise \(\hat{M}G_m\rightrightarrows MG_m\).
\fi
Let \(\Delta(X)=X\otimes 1 +1\otimes X\). 
For later use we state
\begin{prop}\label{prop:binom}
The following binomial identity holds:
\bas
\sum_{i+j=p} \binom{m-i}{m-p} \binom{n-j}{n-p}=\binom{m+n-p+1}{p}.
\eas
\end{prop}
\begin{proof}
Cf. \cite{rationalCGC2018}.
\end{proof}
\begin{defn}
We define the \(p\)th transvectant of \(v^m \otimes w^{n}\), \(\Join^{m+n-2p}: V_m\otimes W_n \rightarrow U_{m-n-2p}\cap \ker M\), as
\bas
\Join^{m+n-2p}v^m \otimes w^{n}=
\sum_{i+j=p}  (-1)^i \binom{p}{i}   \frac{v^{(m)}_{i}}{\binom{m}{i}}\otimes \frac{w^{(n)}_{j}}{\binom{n}{j}}
%\otimes \frac{x^{(m+n-2p)}_{l+k} }{\binom{m+n-2p}{l+k}}
\eas
This definition immediately follows from the symbolic method.
Alternative definitions are also in use, with multiplication constants depending on \(m,n,p\), cf Remark \ref{rem:trans}.
\end{defn}
\iffalse
\begin{defn}
We identify \(\binom{m}{k} u_1^{m-k} u_2^k \rightrightarrows u_k^{(m)}\).
\bas
\lefteqn{\hat{\Join}^{m+n-2p}v^m \otimes w^{n}=(v_1w_2-v_2w_1)^p (v_1x_1+v_2 x_2)^{m-p}(w_1 x_1 + w_w x_2)^{n-p}}&&
\\&=&\sum_{i=0}^p \sum_{l=0}^{m-p} \sum_{k=0}^{n-p} (-1)^i \binom{p}{i}  \binom{m-p}{l} \binom{n-p}{k}  v_1^{m-i-l}v_2^{l+i} w_1^{n-p-k+i} w_2^{k+p-i} x_1^{m-l+n-k-2p}  x_2^{l+k} 
%\\&=&\sum_{i=0}^p (-1)^i \binom{p}{i} v_1^{m-i} v_2^{i} w_1^{i-p +n} w_2^{p-i}
\\&\rightrightarrows&
\sum_{i=0}^p \sum_{l=0}^{m-p} \sum_{k=0}^{n-p} (-1)^i \binom{p}{i}  \binom{m-p}{l} \binom{n-p}{k} \frac{v^{(m)}_{l+i}}{\binom{m}{l+i}}\otimes \frac{w^{(n)}_{k+p-i}}{\binom{n}{k+p-i}}\otimes \frac{x^{(m+n-2p)}_{l+k} }{\binom{m+n-2p}{l+k}}
\eas
\begin{rem}
Compare this with the line arrangements in \cite{frenkel2010categorifying}.
\end{rem}
We now define \(\Join^{(m+n-2p)}_{d}v^m\otimes w^n\) as the coefficient of \(x_d^{(m+n-2p)}\) in \(\hat{\Join}^{m+n-2p}v^m \otimes w^{n}\).
Since the expression \(\hat{\Join}^{m+n-2p}v^m \otimes w^{n}\) is by definition an \(\mathfrak{sl}_2\)-invariant,
the \(\Join^{(m+n-2p)}_{d}v^m\otimes w^n\) form an irreducible \(\mathfrak{sl}_2\) representation, dual do the representation spanned by the \(x_d^{(m+n-2p)}\).
Let \(v^{(m)}_{l+i} w^{(n)}_{k+p-i}=X[k+p-i] \) and \(x^{(m+n-2p)}_{l+k}=Y[l+k]\).
From this formula one can read off \(\Join^{(m+n-2p)}_{d}\) as expressed in the \(v^{(m)}_{l+i}\otimes w^{(n)}_{k+p-i}\), but also 
\(v^{(m)}_{l+i}\otimes w^{(n)}_{k+p-i}\) as expressed in the  \(\Join^{(m+n-2p)}_{d}\).
\end{defn}
\fi
\iffalse
\begin{exm}
Let \(p=0\):
\bas
\hat{\Join}^{m+n}v^m \otimes w^{n}
&=&\sum_{l=0}^{m} \sum_{k=0}^{n} \frac{ 1}{\binom{m+n}{l+k}} v^{(m)}_{l}\otimes w^{(n)}_{k}\otimes x^{(m+n)}_{l+k}
\eas
If we take the inner product with \(x^{(m+n)}_0\) we obtain \(v^{m}\otimes w^{n}\), which indeed equals \(\Join^{m+n} v^{m}\otimes w^{n}\).
If we take the inner product with \(x^{(m+n)}_d\) we obtain 
\bas
\sum_{l=0}^{m} \sum_{k=0}^{n}  v^{(m)}_{l}\otimes w^{(n)}_{k} \delta_{d,l+k}&=&\sum_{l=0}^{m} \sum_{k=0}^{n}\frac{1}{l!k!}  v^{m}_{l}\otimes w^{n}_{k} \delta_{d,l+k}
\\&=&\frac{1}{d!}\sum_{l=0}^{m} \sum_{k=0}^{n}\binom{d}{l}  v^{m}_{l}\otimes w^{n}_{k} \delta_{d,l+k}
\\&=&\frac{1}{d!}\Delta^d(N) v^{m}\otimes w^{n},
\eas
which indeed equals \(\Join^{(m+n)}_d v^{m}\otimes w^{n}\).
\end{exm}
\fi
\iffalse
In general. if we take the inner product with \(x^{(m+n-2q)}_d\) we obtain
\bas
\sum_{i=0}^p \sum_{l=0}^{m-p} \sum_{k=0}^{n-p} (-1)^i\frac{ \binom{p}{i}  \binom{m-p}{l} \binom{n-p}{k}}{\binom{m}{l+i}\binom{n}{k+p-i}} v^{(m)}_{l+i}\otimes w^{(n)}_{k+p-i}
\delta_{p,q} \delta_{d,k+l} \|\Join^{(m+n-2p)} v^{m}\otimes w^{n}\|^2
\eas
MARK
as compared to our original formula
\bas
\Join^{(m+n-2p)}_k v^m \otimes w^n&=&
\sum_{r=0}^k \sum_{i=0}^p (-1)^i \frac{\binom{p}{i}\binom{i+k-r}{k-r} \binom{p-i+r}{r}}{\binom{m}{i}\binom{n}{p-i}}  v_{i+k-r}^{(m)} \otimes w_{p-i+r}^{(n)}
%\\&=&
% i=I-k+r --- I=i+k-r -- J=p+k-I
%\sum_{r=0}^k \sum_{I=k-r}^{k-r+p} (-1)^{I-k+r} \frac{\binom{p}{I-k+r}}{\binom{m}{I-k+r}\binom{n}{p+k-I-r}} \binom{I}{k-r} \binom{p+k-I}{r} v_{I}^{(m)} \otimes w_{p+k-I}^{(n)}
%\\&=&
% i=I-k+r --- I=i+k-r -- J=p+k-I r+q=k
%\sum_{i+j=k+p}\sum_{r+q=k} (-1)^{i-k+r} \frac{\binom{p}{i-q}\binom{i}{q} \binom{j}{r}}{\binom{m}{i-q}\binom{n}{j-r}}  v_{i}^{(m)} \otimes w_{j}^{(n)}
\eas
\begin{exm}
Let \(p=1\).
\bas
\lefteqn{\hat{\Join}^{m+n-2}v^m \otimes w^{n}=}&&
\\&\rightrightarrows&
\sum_{i=0}^1 \sum_{l=0}^{m-1} \sum_{k=0}^{n-1} (-1)^i \frac{\binom{m-1}{l} \binom{n-1}{k}}{\binom{m}{l+i}\binom{n}{k+1-i}\binom{m+n-2}{l+k}} v^{(m)}_{l+i}\otimes w^{(n)}_{k+1-i}\otimes x^{(m+n-2)}_{l+k} 
\\&=&
 \sum_{l=0}^{m-1} \sum_{k=0}^{n-1}  \frac{\binom{m-1}{l} \binom{n-1}{k}}{\binom{m+n-2}{l+k}}\left(\frac{v^{(m)}_{l}}{\binom{m}{l}}\otimes\frac{ w^{(n)}_{k+1}}{\binom{n}{k+1}}
-\frac{v^{(m)}_{l+1}}{\binom{m}{l+1}}\otimes\frac{ w^{(n)}_{k}}{\binom{n}{k}}\right)\otimes x^{(m+n-2)}_{l+k} 
\\&=&
 \sum_{l=0}^{m-1} \sum_{k=0}^{n-1} \frac{1}{mn} \left((m-l)v^{(m)}_{l}\otimes(k+1)  w^{(n)}_{k+1}
%\right. \\&-&\left.
-(l+1) v^{(m)}_{l+1}\otimes (n-k) w^{(n)}_{k}\right)\otimes \frac{x^{(m+n-2)}_{l+k} }{\binom{m+n-2}{l+k}}
\eas
\end{exm}
\fi
\begin{rem}\label{rem:trans}
We compare the definition given in \cite{SVM2007} with the present definition of transvectant:
\bas
(v,w)^{(p)}&=& p! \sum_{i+j=p} (-1)^i \binom{m-i}{p-i}\binom{n-j}{p-j} v_i^m \otimes w_j^n
\\&=& \frac{1}{(m-p)!(n-p)!}\sum_{i+j=p} (-1)^i \frac{\binom{p}{i}}{\binom{m}{i}\binom{n}{j}}   v_i^{(m)} \otimes w_j^{(n)} .
\\&=&\frac{1}{(m-p)!(n-p)!}
\Join^{m+n-2p} v^{m}\otimes w^{n}.
\eas
\end{rem}
\begin{lem}
In order to implement the procedure given in \cite{kassel2012quantum} correctly we compute
\bas
\|\Join^{m+n-2p} v^m \otimes w^n\|^2&=&
\|v^m\otimes w^n\|^2 \frac{\binom{m+n-p+1}{p}}{\binom{m}{p}\binom{n}{p}}.
\eas
\end{lem}
\begin{proof}
\iffalse
We now define the transvectant using the symbolic method: \(A=\hat{\Join}^{m+n-2p}v^m \otimes w^{n}:=[vw]^p(vx)^{m-p}(wx)^{n-p}=(v_1w_2-v_2w_1)^p(v_1x_1+v_2x_2)^{m-p}(w_1x_1+w_2x_2)^{n-p}\)
corresponds to our 
\(\Join^{m+n-2p} v^{m}\otimes w^{n}\) when evaluated at \(x_1=1,x_2=0\), that is, 
\bas
\Join^{m+n-2p}v^m \otimes w^{n}&=&(v_1w_2-v_2w_1)^p v_1^{m-p}w_1^{n-p}
\\&=&\sum_{i=0}^p (-1)^i \binom{p}{i} (v_1w_2)^{p-i} (v_2w_1)^i v_1^{m-p}w_1^{n-p}
\\&=&\sum_{i=0}^p (-1)^i \binom{p}{i} v_1^{m-i} v_2^{i} w_1^{i-p +n} w_2^{p-i}
\\&\rightrightarrows&\sum_{i=0}^p (-1)^i \frac{\binom{p}{i}}{\binom{m}{i}\binom{n}{p-i}}  v_{i}^{(m)} \otimes w_{p-i}^{(n)}.
\eas
\begin{cor}
Notice that, since it is evaluated at \(x_2=0\), the expression is automatically in \(\ker\hat{M}\) as long as we do not evaluate \(x_1=1\),
and therefore \(\Join^{m+n-2p} v^{m}\otimes w^{n}\in\ker\Delta(M)\). The \(\Delta(H)\)-eigenvalue equals the power of \(x_1\), that is \(m+n-2p\).
\end{cor}
\fi
\iffalse
It then follows that
\bas
\Join^{m+n-2p}_k v^m \otimes w^{n}&=&\frac{1}{k!} (v_1\frac{\partial}{\partial v_2}+w_1\frac{\partial}{\partial w_2})^k (v_1w_2-v_2w_1)^p v_1^{m-p}w_1^{n-p}
\\&=&\frac{1}{k!} \sum_{r=0}^k \binom{k}{r} v_1^r w_1^{k-r} \frac{\partial^{k-r}}{\partial v_2^{k-r}}\frac{\partial^{r}}{\partial w_2^{r}}\sum_{i=0}^p (-1)^i \binom{p}{i} (v_1w_2)^{p-i} (v_2w_1)^i v_1^{m-p}w_1^{n-p}
\\&=&\frac{1}{k!} \sum_{r=0}^k \binom{k}{r} \sum_{i=0}^p (-1)^i \frac{i!}{(i-k+r)!}\frac{(p-i)!}{(p-i-r)!}\binom{p}{i} v_1^{m-i+k-r} v_2^{i-k+r} w_1^{i-p +n+r} w_2^{p-i-r}
\\&\rightrightarrows&\frac{\binom{m+n-2p}{k}}{k!(??)}\sum_{i=0}^p (-1)^i \frac{\binom{p}{i}}{\binom{m}{i-k+r}\binom{n}{p-i-r}} \frac{i!}{(i-k+r)!}\frac{(p-i)!}{(p-i-r)!} v_{i-k+r}^{(m)} \otimes w_{p-i-r}^{(n)}.
\eas
\fi
One has
\bas
\lefteqn{(\Join^{m_1+n_1-2p_1} v^{m_1}\otimes w^{n_1},\Join^{m_2+n_2-2p_2} v^{m_2}\otimes w^{n_2})=}&&\\&=&\sum_{i_1=0}^{p_1}\sum_{i_2=0}^{p_2} (-1)^{i_1+i_2} 
\frac{\binom{{p_1}}{i_1}}{\binom{m_1}{i_1}\binom{n_1}{p_1-i_1}}\frac{\binom{{p_2}}{i_2}}{\binom{m_2}{i_2}\binom{n_2}{p_2-i_2}} 
(v_{i_1}^{(m_1)},v_{i_2}^{(m_2)})_{V_m}(w_{p_1-i_1}^{(n_1)},w_{p_2-i_2}^{(n_2)})_{W_n}
\\&=&\delta_{p_1,p_2}\delta_{m_1,m_2}\delta_{n_1,n_2}
\sum_{i=0}^{p} \frac{\binom{{p}}{i}^2}{\binom{m}{i}\binom{n}{p-i}}  \|v^m\|^2 \|w^n\|^2
\eas
and it follows that the transvectants are orthogonal and that
\bas
\|\Join^{m+n-2p} v^{m}\otimes w^{n}\|^2&=&\|v^m\|^2 \|w^n\|^2\sum_{i=0}^p \frac{\binom{p}{i}^2}{\binom{m}{i}\binom{n}{p-i}}
\\&=&\|v^m\|^2 \|w^n\|^2\frac{p!^2}{m!n!}\sum_{i=0}^p \frac{ (m-i)!  (n-p+i)! }{i!(p-i)!}
\eas
Using Proposition \ref{prop:binom}
we find
\bas
\sum_{i+j=p} \frac{ (m-i)!  (n-j)! }{i!j!} &=&\sum_{i+j=p} \binom{m-i}{m-p}\binom{n-j}{n-p} \frac{ (m-p)! (p-i)! (n-p)! (p-j)!}{i!j!}
\\&=& (m-p)!  (n-p)! \sum_{i+j=p} \binom{m-i}{m-p}\binom{n-j}{n-p}
\\&=& (m-p)!  (n-p)! \binom{m+n-p+1}{p}
\eas
%\begin{proof}
and it follows that
\bas
\|\Join^{m+n-2p} v^m \otimes w^n\|^2&=&\|v^m\|^2 \|w^n\|^2\frac{p!^2}{m!n!}\sum_{i=0}^p \frac{ (m-i)!  (n-p+i)! }{i!(p-i)!}
\\&=&\|v^m\|^2 \|w^n\|^2\frac{p!(m-p)!}{m!} \frac{p! (n-p)!}{n!} \binom{m+n-p+1}{p}
\\&=&\|v^m\|^2 \|w^n\|^2\frac{\binom{m+n-p+1}{p}}{\binom{m}{p}\binom{n}{p}}.
\eas
\end{proof}
\begin{cor}
\bas
\|\Join^{(m+n-2p)}_k v^m \otimes w^n\|^2&=&
\|v^m\otimes w^n\|^2 \frac{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}{\binom{m}{p}\binom{n}{p}}
\eas
\end{cor}
\iffalse
\begin{exm}
Take \(p=1\). Then \(\|\Join^{m+n-2} v^{m}\otimes w^{n}\|^2=\frac{m+n}{mn}\) if we assume the basis vectors in \(\ker M\) to have length \(1\).
In fact, \(\Join^{m+n-2}v^m \otimes w^n=\sum_{i=0}^1 (-1)^i \frac{1}{\binom{m}{i}\binom{n}{1-i}}  v_{i}^{(m)} \otimes w_{1-i}^{(n)}= \frac{1}{n}  v^{(m)} \otimes w_{1}^{(n)}-\frac{1}{m}  v_{1}^{(m)} \otimes w^{(n)} \). Thus \(\|\Join^{m+n-2}v^m \otimes w^n\|^2=\frac{1}{n^2}n+\frac{1}{m^2}m=\frac{m+n}{mn}\), as predicted by the general formula.
\end{exm}
\fi
\iffalse
\begin{exm}
We compute \(\Join^{(m+n)}_1 v^m \otimes w^n\) and \(\Join^{(m+n-2)}v^m \otimes w^n\).
\bas
\Join^{(m+n)}_1 v^m \otimes w^n&=& v^{(m)} \otimes w_{1}^{(n)}+v_{1}^{(m)} \otimes w^{(n)}\\
\Join^{(m+n-2)}v^m \otimes w^n&=& \frac{1}{n}  v^{(m)} \otimes w_{1}^{(n)}-\frac{1}{m}  v_{1}^{(m)} \otimes w^{(n)}
\eas
The matrix is
\bas
A_{[1]}=\begin{pmatrix} 1&1\\ \frac{1}{n} & -\frac{1}{m} \end{pmatrix}
\eas
To compute the transpose, we multiply the first column with \(\|w_{1}^{(n)}\|^2=n\) and the second column with \(\|v_{1}^{(m)}\|^2=m\)
and we divide the first row by \(\|\Join^{m+n}_1 v^m \otimes w^n\|^2=m+n\) and the second row by \(\|\Join^{m+n-2}v^m \otimes w^n\|^2=\frac{m+n}{mn}\).
Then we take the ordinary matrix transpose.
\bas
A_{[1]}^\perp=\frac{1}{n+m}\begin{pmatrix} n&nm\\ m & -nm \end{pmatrix}
\eas
and we check that \(A_{[1]}^\perp=A_{[1]}^{-1}\).
\end{exm}
\fi
\iffalse
\begin{exm}
We compute \(\Join^{(m+n)}_2 v^m \otimes w^n\), \(\Join^{(m+n-2)}_1 v^m \otimes w^n\) and  \(\Join^{(m+n-4)} v^m \otimes w^n\).
\bas
\Join^{(m+n)}_2 v^m \otimes w^n&=& v^{(m)} \otimes w_{2}^{(n)}+v_{1}^{(m)} \otimes w_{1}^{(n)}+  v_{2}^{(m)} \otimes w^{(n)} \\
\Join^{(m+n-2)}_1 v^m \otimes w^n&=& \frac{2}{n}  v^{(m)} \otimes w_{2}^{(n)}-\frac{1}{m}  v_{1}^{(m)} \otimes w_1^{(n)}+\frac{1}{n}  v_1^{(m)} \otimes w_{1}^{(n)}-2\frac{1}{m}  v_{2}^{(m)} \otimes w^{(n)}\\
\Join^{(m+n-4)} v^m \otimes w^n&=&
\frac{1}{\binom{n}{2}}  v^{(m)} \otimes w_{2}^{(n)}
- \frac{2}{mn}  v_{1}^{(m)} \otimes w_{1}^{(n)}
+ \frac{1}{\binom{m}{2}}  v_{2}^{(m)} \otimes w^{(n)}
\eas
and
\bas
A_{[2]}=\begin{pmatrix} 1&1&1\\ \frac{2}{n} & \frac{1}{n}-\frac{1}{m}&-\frac{2}{m}\\\frac{1}{\binom{n}{2}} &- \frac{2}{mn} &\frac{1}{\binom{m}{2}}  \end{pmatrix}
\eas
We then multiply the first column by \(\binom{n}{2}\), the second by \(mn\) and the third by \(\binom{m}{2}\).
Then we divide the first row by \(\binom{m+n}{2}\), the second by \(\frac{m+n}{mn}(m+n-2)\) and the third by \(\frac {\binom{m+n-1}{2}}{\binom{m}{2}\binom{n}{2}}\)
Finally we take the ordinary matrix transpose. 
This is better left to Maple.
\end{exm}
\fi
Although we have already computed \(\|\Join^{(m+n-2p)}_k v^m \otimes w^n\|^2\),
we have not computed \(\Join^{(m+n-2p)}_k v^m \otimes w^n\) itself.
We give here an explicit derivation, but mention that it also immediately follows from the symbolic method.
\bas
\Join^{(m+n-2p)}_k v^m \otimes w^n&=&\frac{1}{k!}\Delta^k(N) \Join^{m+n-2p} v^{m}\otimes w^{n}
\\&=&
\frac{1}{k!}\Delta^k(N) 
\sum_{i=0}^p (-1)^i \frac{\binom{p}{i}}{\binom{m}{i}\binom{n}{p-i}}  v_{i}^{(m)} \otimes w_{p-i}^{(n)}
\\&=&
\frac{1}{k!}
\sum_{r=0}^k \sum_{i=0}^p (-1)^i \frac{\binom{p}{i}}{\binom{m}{i}\binom{n}{p-i}} \binom{k}{r} \frac{(i+k-r)!}{i!}\frac{(p-i+r)!}{(p-i)!} v_{i+k-r}^{(m)} \otimes w_{p-i+r}^{(n)}
\\&=&
\sum_{r=0}^k \sum_{i=0}^p (-1)^i \frac{\binom{p}{i}}{\binom{m}{i}\binom{n}{p-i}} \binom{i+k-r}{k-r} \binom{p-i+r}{r} v_{i+k-r}^{(m)} \otimes w_{p-i+r}^{(n)}
\\&=&
% i=I-k+r --- I=i+k-r -- J=p+k-I
\sum_{r=0}^k \sum_{I=k-r}^{k-r+p} (-1)^{I-k+r} \frac{\binom{p}{I-k+r}}{\binom{m}{I-k+r}\binom{n}{p+k-I-r}} \binom{I}{k-r} \binom{p+k-I}{r} v_{I}^{(m)} \otimes w_{p+k-I}^{(n)}
\\&=&
% i=I-k+r --- I=i+k-r -- J=p+k-I r+q=k
\sum_{i+j=k+p}\sum_{r+q=k} (-1)^{i-k+r} \frac{\binom{p}{i-q}\binom{i}{q} \binom{j}{r}}{\binom{m}{i-q}\binom{n}{j-r}}  v_{i}^{(m)} \otimes w_{j}^{(n)}
\eas
In all formulas the summation convention is such that for a binomial expression we must have that the numbers \(a\) and \( b\) in \(\binom{a}{b}\) are natural numbers (zero included)
with \(a\geq b\).
\begin{defn}
Define the Clebsch-Gordan coefficient (CGC), also known as \(3j\)-symbol , by
\[\begin{pmatrix} m& n& m+n-2p\\i&j& k\end{pmatrix}=\sum_{r+q=k} (-1)^{i-k+r} \frac{\binom{p}{i-q}\binom{i}{q} \binom{j}{r}}{\binom{m}{i-q}\binom{n}{j-r}}, \quad i+j=p+k\]
with \(j_1=m, j_2=n\) and \(j_3=n+m-2p\) as the \(3j\)'s. 
\end{defn}
\begin{lem}
The \(3j\)-symbols are orthogonal:
\bas
\lefteqn{\sum\begin{pmatrix} {m_1}& {n_1}& {m_1}+{n_1}-2p_1\\i_1&j_1& k_1\end{pmatrix}
\begin{pmatrix} {m_2}& {n_2}& {m_2}+{n_2}-2p_2\\i_2&j_2& k_2\end{pmatrix} \binom{{m_1}}{i_1} \binom {{n_1}}{j_1}}&&
\\&=&
\delta_{k_1,k_2}\delta_{m_1,m_2}\delta_{n_1,n_2} \binom{m_1+n_1-2p_1}{k_1}
\|v^{m_1}\otimes w^{n_1}\|^2 \frac{\binom{m_1+n_1-p_1+1}{p_1}}{\binom{m_1}{p_1}\binom{n_1}{p_1}}
\eas
where the summation is over \(i_1+j_1=p_1+k_1=p_2+k_2=i_2+j_2.\)
\end{lem}
\begin{proof}
We compute \((\Join^{(m_1+n_1-2p_1)}_{k_1} v^{m_1}\otimes  w^{n_1},  \Join^{(m_2+n_2-2p_2)}_{k_2} v^{m_2}\otimes  w^{n_2} )_{V\otimes V}\).
\bas
\lefteqn{(\Join^{(m_1+n_1-2p_1)}_{k_1} v^{m_1}\otimes  w^{n_1} , \Join^{(m_2+n_2-2p_2)}_{k_2} v^{m_2}\otimes  w^{n_2} )_{V\otimes V}=}&&
\\&=&
\delta_{k_1,k_2} \binom{m_1+n_1-2p_1}{k_1}(\Join^{(m_1+n_1-2p_1)} v^{m_1}\otimes  w^{n_1} , \Join^{(m_2+n_2-2p_2)} v^{m_2}\otimes  w^{n_2} )_{\ker\Delta(M)}
\\&=&
\delta_{k_1,k_2}\delta_{m_1,m_2}\delta_{n_1,n_2}  \binom{m_1+n_1-2p_1}{k_1}
\|v^{m_1}\otimes w^{n_1}\|^2 \frac{\binom{m_1+n_1-p_1+1}{p_1}}{\binom{m_1}{p_1}\binom{n_1}{p_1}}
\eas
\end{proof}
\begin{thm}[Rational Clebsch-Gordan Coefficients]\label{thm:RCGC}

The inversion formula to the definition of \(\Join^{(m+n-2p)}_{k}v^m\otimes v^n\) is
\bas
v^{(m)}_i\otimes v^{(n)}_j&=&\sum_{p+k=i+j}\begin{pmatrix} m&n&m+n-2p\\i&j&k\end{pmatrix}\frac{ \binom{m}{i}\binom{n}{j}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes v^n.
\eas
\end{thm}
\begin{rem}\label{rem:pis0}
We compute the special case \(p=0\).
\[\begin{pmatrix} m& n& m+n\\i&j& i+j\end{pmatrix}=\sum_{r+q=i+j} (-1)^{-j+r} \frac{\binom{0}{i-q}\binom{i}{q} \binom{j}{r}}{\binom{m}{i-q}\binom{n}{j-r}}=1,\]
since \(i-q+j-r=0\), and therefore \(q=i\) and \(r=j\).
\end{rem}
\begin{rem}
This theorem, or variants of it, is well known in quantum mechanics, and in the context of quantum groups.
In the context in which we plan to use it, we have no previous examples of its use.
\end{rem}
\begin{proof}
We consider the equation
\[
A_{[r]}\mathbf{x}=\mathbf{y}
\]
where 
\[
\mathbf{y}=\begin{pmatrix} 
\Join^{(m+n)}_r v^m\otimes v^n \\
\Join^{(m+n-2)}_{r-1} v^m\otimes v^n \\
\vdots
\\
\Join^{(m+n-2r+2)}_1 v^m\otimes v^n \\
\Join^{m+n-2r} v^m\otimes v^n 
\end{pmatrix}
\]
and
\[
\mathbf{x}=\begin{pmatrix}
v^{m}\otimes w^{(n)}_r\\
v^{(m)}_1\otimes w^{(n)}_{r-1}\\
\vdots\\
v^{(m)}_{r-1}\otimes w^{(n)}_1\\
v^{(m)}_r\otimes w^n\\
\end{pmatrix}
\]
We first make this into an orthonormal set (orthogonality is clear from the definition of the inner product) by dividing each and every term in \(x\) and \(y\) by its norm.
Thus the \(i+1\)st column of \(A_{[r]}\) get multiplied by the \(\|v^{(m)}_i\otimes w^{(n)}_{r-i}\|\)
and the \(p+1\)st row divided by \(\|\Join^{(m+n-2p)}_{r-p} v^m\otimes v^n\|\).
The resulting matrix is then transposed and we go back to the original bases by doing the same thing again (this is because
the roles of \(x\) and \(y\) are now switched, and therefore multiplication is switched with division).
We recall that \(\|v^{(m)}_i\otimes w^{(n)}_{j}\|^2=\binom{m}{i}\binom{n}{j}\|v^m\otimes w^n\|^2\) and \(\|\Join^{(m+n-2p)}_{k} v^m\otimes v^n\|^2=\|v^m\otimes w^n\|^2 \frac{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}{\binom{m}{p}\binom{n}{p}}
\), with \(i+j=p+k=r\).
\end{proof}
\begin{rem}
Nice as this inversion formula for the Clebsch-Gordan coefficients may look, the reader should realize that the right hand side contains expressions that are computable,
but may not always have a nice general formula. On the bright side we notice that in the normal form computations we often need special cases with very simple \(3j\)-symbols.
In physics problems, it would seem the finite dimensional results are enough,
but in the computation of the structure constants of the Lie algebra of polynomial vector fields with a basis consisting of \(N\)-orbits, we need general formulas.
\end{rem}
\iffalse
\begin{exm}
We construct \(A_{[2]}^{-1}\) from the inversion formula:
\bas
v^{(m)}_i\otimes w^{(n)}_j&=&\sum_{p+k=i+j=2}\begin{pmatrix} m&n&m+n-2p\\i&j&k\end{pmatrix}\frac{ \binom{m}{i}\binom{n}{j}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes w^n.
\eas
\bas
v^{(m)}\otimes w^{(n)}_2&=&\sum_{p+k=2}\begin{pmatrix} m&n&m+n-2p\\0&2&k\end{pmatrix}\frac{\binom{n}{2}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes w^n.
\\&=& 
\begin{pmatrix} m&n&m+n\\0&2&2\end{pmatrix}\frac{\binom{n}{2}}{\binom{m+n}{2}}\Join^{(m+n)}_{2}v^m\otimes w^n
\\&+&\begin{pmatrix} m&n&m+n-2\\0&2&1\end{pmatrix}\frac{\binom{n}{2}mn}{(m+n-2)(m+n)}\Join^{(m+n-2)}_{1}v^m\otimes w^n
\\&+&\begin{pmatrix} m&n&m+n-4\\0&2&0\end{pmatrix}\frac{\binom{n}{2}\binom{m}{2}\binom{n}{2}}{\binom{m+n-1}{2}}\Join^{(m+n-4)}v^m\otimes w^n
\eas
\bas
v^{(m)}_1\otimes w^{(n)}_1&=&\sum_{p+k=2}\begin{pmatrix} m&n&m+n-2p\\1&1&k\end{pmatrix}\frac{ mn\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes w^n
\\&=&
\begin{pmatrix} m&n&m+n\\1&1&2\end{pmatrix}\frac{ mn}{\binom{m+n}{2}}\Join^{(m+n)}_{2}v^m\otimes w^n
\\&+&
\begin{pmatrix} m&n&m+n-2\\1&1&1\end{pmatrix}\frac{ m^2n^2}{\binom{m+n-2}{1}\binom{m+n}{1}}\Join^{(m+n-2)}_{1}v^m\otimes w^n
\\&+&
\begin{pmatrix} m&n&m+n-4\\1&1&0\end{pmatrix}\frac{ mn\binom{m}{2}\binom{n}{2}}{\binom{m+n-4}{0}\binom{m+n-1}{2}}\Join^{m+n-4}v^m\otimes w^n
\eas
\bas
v^{(m)}_2\otimes w^{(n)}&=&\sum_{p+k=2}\begin{pmatrix} m&n&m+n-2p\\2&0&k\end{pmatrix}\frac{ \binom{m}{2}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes w^n.
\\&=&
\begin{pmatrix} m&n&m+n\\2&0&2\end{pmatrix}\frac{ \binom{m}{2}}{\binom{m+n}{2}}\Join^{(m+n)}_{2}v^m\otimes w^n
\\&+&\begin{pmatrix} m&n&m+n-2\\2&0&1\end{pmatrix}\frac{ \binom{m}{2}mn}{\binom{m+n-2}{1}(m+n)}\Join^{(m+n-2)}_{1}v^m\otimes w^n
\\&+&\begin{pmatrix} m&n&m+n-4\\2&0&0\end{pmatrix}\frac{ \binom{m}{2}\binom{m}{2}\binom{n}{2}}{(m+n-1)}\Join^{m+n-4}v^m\otimes w^n.
\eas
The definition of the \(3j\)-symbol is
\[\begin{pmatrix} m& n& m+n-2p\\i&j& k\end{pmatrix}=\sum_{r+q=k} (-1)^{i-k+r} \frac{\binom{p}{i-q}\binom{i}{q} \binom{j}{r}}{\binom{m}{i-q}\binom{n}{j-r}}, \quad i+j=p+k\]
that is,
\[\begin{pmatrix} m& n& m+n-2p\\2&0& k\end{pmatrix}= (-1)^{2-k} \frac{\binom{2}{k}}{\binom{m}{2-k}}, \]
\[\begin{pmatrix} m& n& m+n-2p\\0&2& k\end{pmatrix}=\sum_{r+q=k} (-1)^{-k+r} \frac{\binom{p}{-q}\binom{0}{q} \binom{2}{r}}{\binom{m}{0-q}\binom{n}{2-r}}=\frac{\binom{2}{k}}{\binom{n}{2-k}}\]
\[\begin{pmatrix} m& n& m+n-2p\\1&1& k\end{pmatrix}=\sum_{q=0}^k (-1)^{1-q} \frac{\binom{p}{1-q}\binom{1}{q} \binom{1}{k-q}}{\binom{m}{1-q}\binom{n}{1-k+q}}\]
This implies
\bas
v^{(m)}_2\otimes w^{(n)}&=&
\frac{ \binom{m}{2}}{\binom{m+n}{2}}\Join^{(m+n)}_{2}v^m\otimes w^n
\\&-&\frac{2 \binom{m}{2}n}{(m+n-2)(m+n)}\Join^{(m+n-2)}_{1}v^m\otimes w^n
\\&+&\frac{\binom{m}{2}\binom{n}{2}}{(m+n-1)}\Join^{m+n-4}v^m\otimes w^n.
\eas
\[\begin{pmatrix} m& n& m+n-4\\1&1& 0\end{pmatrix}= - \frac{2}{mn}\]
\[\begin{pmatrix} m& n& m+n-2\\1&1& 1\end{pmatrix}
=\sum_{q=0}^1 (-1)^{1-q} \frac{1}{\binom{m}{1-q}\binom{n}{q}}
=
\frac{1}{n}
- \frac{1}{m}
\]
\[
\begin{pmatrix} m& n& m+n\\1&1& 2\end{pmatrix}=1
\]
We now have
\bas
v^{(m)}_1\otimes w^{(n)}_1&=&
\frac{ mn}{\binom{m+n}{2}}\Join^{(m+n)}_{2}v^m\otimes w^n
\\&+&
\frac{ mn(m-n)}{(m+n-2)(m+n)}\Join^{(m+n-2)}_{1}v^m\otimes w^n
\\&-&
\frac{ 2\binom{m}{2}\binom{n}{2}}{\binom{m+n-1}{2}}\Join^{m+n-4}v^m\otimes w^n
\eas

We find
\bas
v^{(m)}\otimes w^{(n)}_2&=&
\frac{\binom{n}{2}}{\binom{m+n}{2}}\Join^{(m+n)}_{2}v^m\otimes w^n
\\&+&\frac{2\binom{n}{2}m}{(m+n-2)(m+n)}\Join^{(m+n-2)}_{1}v^m\otimes w^n
\\&+&\frac{\binom{n}{2}\binom{m}{2}}{\binom{m+n-1}{2}}\Join^{(m+n-4)}v^m\otimes w^n
\eas
We find
\bas
\begin{pmatrix} v^{m} \otimes w^{(n)}_2 \\ v^{(m)}_1\otimes w^{(n)}_1 \\ v^{(m)}_2 \otimes w^n\end{pmatrix}
&=&\begin{pmatrix}\frac{\binom{n}{2}}{\binom{m+n}{2}} &\frac{2\binom{n}{2}m}{(m+n-2)(m+n)}&\frac{\binom{n}{2}\binom{m}{2}}{\binom{m+n-1}{2}} \\
\frac{ mn}{\binom{m+n}{2}} &\frac{ mn(m-n)}{(m+n-2)(m+n)}&-\frac{ 2\binom{m}{2}\binom{n}{2}}{\binom{m+n-1}{2}} \\
\frac{ \binom{m}{2}}{\binom{m+n}{2}} &-\frac{2 \binom{m}{2}n}{(m+n-2)(m+n)}&\frac{\binom{m}{2}\binom{n}{2}}{(m+n-1)} \end{pmatrix}
\begin{pmatrix} \Join^{(m+n)}_2 v^m \otimes w^n  \\ \Join^{(m+n-2)}_1 v^m \otimes w^n \\ \Join^{m+n-4}v^m \otimes w^n \end{pmatrix}
\eas
MARK
\end{exm}
\fi
\iffalse
\begin{exm}
	\bas
	\begin{pmatrix}
		v^m\otimes w^{{(n)}}_2\\
		v^{(m)}_1\otimes w^{(n)}_{1}\\
		v^{(m)}_2\otimes w^n\\
	\end{pmatrix}=\left[ \begin {array}{ccc} {\frac {n \left( n-1 \right) }{ \left( n+m
			-1 \right)  \left( n+m \right) }}&{\frac {n \left( n-1 \right) m}{
			\left( n+m-2 \right)  \left( n+m \right) }}&\frac{1}{2}\,{\frac {m \left( m-1
			\right) n \left( n-1 \right) }{ \left( n+m-2 \right)  \left( n+m-1
			\right) }}\\ \noalign{\medskip}\,{2\frac {nm}{ \left( n+m-1 \right) 
			\left( n+m \right) }}&{\frac {nm \left( m-n \right) }{ \left( n+m-2
			\right)  \left( n+m \right) }}&-{\frac {m \left( m-1 \right) n
			\left( n-1 \right) }{ \left( n+m-2 \right)  \left( n+m-1 \right) }}
	\\ \noalign{\medskip}{\frac {m \left( m-1 \right) }{ \left( n+m-1
			\right)  \left( n+m \right) }}&-{\frac {m \left( m-1 \right) n}{
			\left( n+m-2 \right)  \left( n+m \right) }}&\frac{1}{2}\,{\frac {m \left( m-1
			\right) n \left( n-1 \right) }{ \left( n+m-2 \right)  \left( n+m-1
			\right) }}\end {array} \right] \begin{pmatrix} 
		\Join^{(m+n)}_2 v^m\otimes v^n \\
		\Join^{(m+n-2)}_{1} v^m\otimes v^n \\
		\Join^{m+n-4} v^m\otimes v^n 
	\end{pmatrix}
	\eas
\end{exm}
\fi
\iffalse
\begin{exm}
NEEDS UPDATE
An example where it is possible to find a general formula for a class of transvectants is the following.
Let in the 3D case \(v^{2p}=z^p\), \(w^{2q}=z^q\).
Then \bas
\Join^{2(p+q-2n)} v^{2p}\cdot v^{2q}&=&(2n)!(n!)^2\binom{2n-p-q-1}{n}\binom{n-p-1}{n}\binom{n-q-1}{n}z^{p+q-2n}\Delta^n\\&=&(2n)!(n!)^2\binom{2n-p-q-1}{n}\binom{n-p-1}{n}\binom{n-q-1}{n}\Delta^n v^{2(p+q-2n)}\eas
and \(\Join^{2(p+q-2n-1)}_{2n+1} v^{2p}\otimes v^{2q}=0\), where \(\Delta=xz-y^2\)
\end{exm}
\fi
\iffalse
\begin{lem}
Let \(v^m,w^n\in\ker M\) with eigenvalues \(m,n\), respectively. Then
\[
\Join^{m+n-2p} v^m\otimes  w^n = \sum_{i+j=p} (-1)^i \binom{m-i}{j}\binom{n-j}{i} v_i^m \otimes w_j^n \in \ker \Delta(M)
\]
with eigenvalue \( m+n-2p\).
\end{lem}
\begin{proof}
\bas
\Delta(M) \Join^{m+n-2p} v^m\otimes  w^n &=& \Delta(M)  \sum_{i+j=p} (-1)^i \binom{m-i}{j}\binom{n-j}{i} v_i^m \otimes w_j^n
\\&=&   \sum_{i+j=p} (-1)^i \binom{m-i}{j}\binom{n-j}{i}M v_i^m \otimes w_j^n
\\&+&   \sum_{i+j=p} (-1)^i \binom{m-i}{j}\binom{n-j}{i} v_i^m \otimes M w_j^n
\\&=&   \sum_{i+j=p} (-1)^i \binom{m-i}{j}\binom{n-j}{i}i(m-i+1) v_{i-1}^m \otimes w_j^n
\\&+&   \sum_{i+j=p} (-1)^i \binom{m-i}{j}\binom{n-j}{i}j(n-j+1) v_i^m \otimes  w_{j-1}^n
\\&=&   -\sum_{i+j=p-1} (-1)^i \binom{m-i-1}{j}\binom{n-j}{i+1}(i+1)(m-i) v_{i}^m \otimes w_j^n
\\&+&   \sum_{i+j=p-1} (-1)^i \binom{m-i}{j+1}\binom{n-j-1}{i}(j+1)(n-j) v_i^m \otimes  w_{j}^n
\\&=&   -\sum_{i+j=p-1} (-1)^i \binom{m-i-1}{j}\binom{n-j-1}{i}(n-j)(m-i) v_{i}^m \otimes w_j^n
\\&+&   \sum_{i+j=p-1} (-1)^i \binom{m-i-1}{j}\binom{n-j-1}{i}(m-i)(n-j) v_i^m \otimes  w_{j}^n
\\&=&0.
\eas
\end{proof}
\fi
\iffalse
\begin{rem}
\newcommand*\pFqskip{8mu}
\catcode`,\active
\newcommand*\pFq{\begingroup
        \catcode`\,\active
        \def ,{\mskip\pFqskip\relax}%
        \dopFq
}
\catcode`\,12
\def\dopFq#1#2#3#4#5{%
        {}_{#1}F_{#2}\biggl[\genfrac..{0pt}{}{#3}{#4};#5\biggr]%
        \endgroup
}
%Change \pFqskip to whatever spacing you want between the elements. You use it like
\( \sum_{i=0}^p\binom{p}{i}^4=\pFq{4}{3}{-p,-p,-p,-p}{\ 1,\ 1,\ 1}{1}\).
\[
\pFq{2}{1}{a,b}{\ c}{1}=\sum_{i=0}^\infty \frac{(a)_i(b)_i}{(c)_i i!}
\]
where
\[
(q)_i=q\cdots(q+i-1)
\]
For instance, \((-p)_{m}=(-p)(-p+1)\cdots(-p+m-1)=(-1)^m p(p-1)\cdots(p-m+1)=(-1)^m \frac{p!}{(p-m)!}\).
\[
\pFq{2}{1}{-p,b}{\ c}{1}=\sum_{i=0}^p (-1)^i\binom{p}{i} \frac{(b)_i}{(c)_i}
\]
\end{rem}
\begin{lem}
\( \| \Join^{m+n-2p} v^m\otimes  w^n\|_{V_m\otimes W_n}=\sqrt{ \sum_{i=0}^p \binom{p}{i}^4} \binom{m}{p}\binom{n}{p} \|v^m\otimes w^n\|_{\ker\Delta(M)}\).
\end{lem}
\begin{proof}
\bas
 \| \Join^{m+n-2p} v^m\otimes  w^n\|_{V_m\otimes W_n}^2&=& \sum_{i+j=p} \binom{m-i}{j}^2\binom{n-j}{i}^2 \binom{m}{i}^2\binom{n}{j}^2 \|v^m\|^2_{\ker M} \|w^n\|^2_{\ker M}
 \\&=&  \frac{(m!)^2}{((m-p)!)^2 (p!)^2}  \frac{(n!)^2}{(p!)^2((n-p)!)^2 }\sum_{i+j=p}\frac{(p!)^4}{(i!)^4(j!)^4}  \|v^m\|^2_{\ker M} \|w^n\|^2_{\ker M}
 \\&=&  \binom{m}{p}^2 \binom{n}{p}^2 \sum_{i=0}^p\binom{p}{i}^4  \|v^m\otimes w^n\|^2_{\ker \Delta(M)}
 \eas
 In the Koornwinder inner product this is, using the \(A_0\)-formula for the transvectant,
\bas
A_0&=&
\sum_{\nu=0}^\lambda (-1)^\nu \frac{\binom{\lambda}{\nu}}{\binom{2j}{\nu}\binom{2j^\prime}{\lambda-\nu}}  u_{\nu}^{(2j)} \otimes v_{\lambda-\nu}^{(2j^\prime)}\otimes  x_0^{(2j+2j^\prime-2\lambda)}
\\&=&
\sum_{i=0}^p (-1)^i \frac{\binom{p}{i}}{\binom{m}{i}\binom{n}{j}}  u_{i}^{(m)} \otimes v_{j}^{(n)}\otimes  x_0^{(m+n-2p)}
\eas
\bas
 \| \Join^{m+n-2p} v^m\otimes  w^n\|_V^2&=& \sum_{i+j=p} \binom{p}{i}^2 \binom{m}{i} \binom{n}{j}\frac{1}{\binom{m}{i}^2\binom{n}{j}^2}
 \\&=&  \sum_{i+j=p} \frac{\binom{p}{i}^2}{\binom{m}{i}\binom{n}{j}}
 \\&=&\frac{p!^2}{m!n!}  \sum_{i=0}^p \frac{(m-i)!(n -p+i)!}{(p-i)!}\frac{1}{i!}
 \\&=&\frac{p!}{m!n!}  \sum_{i=0}^p \binom{p}{i}(m-i)!(n -p+i)!
 \eas
\end{proof}
\fi
\iffalse
Then
\bas
\Delta^k(N)\Join^{m+n-2p} v^m\otimes  w^n &=&
\sum_{i+j=p} (-1)^i\sum_{r+q=k} \binom{m-i}{j}\binom{n-j}{i}\binom{k}{r}  v_{i+r}^m \otimes w_{j+q}^n \\
&=&\sum_{i+j=p+k}\sum_{r=0}^k (-1)^{i-r}\binom{m-i+r}{m-p}\binom{n+i-r-p}{n-p}\binom{k}{r}  v_{i}^m \otimes w_{j}^n .
\eas
We write \(\Join^{m+n-2p}_k v^m\otimes  w^n\) for \(\Delta^k(N)\Join^{m+n-2p} v^m\otimes  w^n\) and \(\Join^{(m+n-2p)}_k v^m\otimes  w^n=\frac{1}{k!}\Join^{m+n-2p}_k v^m\otimes  w^n\).
Define  \(\begin{pmatrix} m& n& m+n-2p\\i&j& k\end{pmatrix}=\sum_{r=0}^k (-1)^{i-r}\binom{m-i+r}{m-p}\binom{n+i-r-p}{n-p}\binom{k}{r} \),
the \(3j\)-symbol (with \(j_1=m, j_2=n\) and \(j_3=n+m-2p\) as the \(3j\)'s). We write
\bas
\Join^{m+n-2p}_k v^m\otimes  w^n &=&\sum_{i+j=p+k}\begin{pmatrix} m& n& m+n-2p\\i&j& k\end{pmatrix}  v_{i}^m \otimes w_{j}^n .
\eas
\fi
\iffalse
\begin{lem}
\(\|\Join^{m+n-2p}_k v^m\otimes  w^n\|=\binom{n+m-2p}{k} \binom{m}{p} \binom{n}{p}\sqrt{ \sum_{i=0}^p\binom{p}{i}^4} \|v^m\otimes w^n\|_{\ker \Delta(M)}\).
\end{lem}
\begin{proof}
\bas
\|\Join^{m+n-2p}_k v^m\otimes  w^n\|&=&\binom{n+m-2p}{k} \|\Join^{m+n-2p} v^m\otimes  w^n\|_{\ker \Delta(M)}
\\&=&\binom{n+m-2p}{k} \binom{m}{p} \binom{n}{p}\sqrt{ \sum_{i=0}^p\binom{p}{i}^4} \|v^m\otimes w^n\|_{\ker \Delta(M)}
\eas
\end{proof}
\begin{cor}
\(\|\Join^{m+n-2p}_k\|=\binom{n+m-2p}{k} \binom{m}{p} \binom{n}{p}\sqrt{ \sum_{i=0}^p\binom{p}{i}^4}\).
\end{cor}
\fi
\iffalse
\begin{lem}
Fix \(p\) and \(k\). The vector \( \Join^{m+n-2p}_k v^m\otimes  w^n \) is a linear combination of vectors of the form \(v_i^{m}\otimes v_{p-i+k}^{n}\).
Therefore, we have
\bas
\begin{pmatrix} m&n&n+m-2p\\i&j&k\end{pmatrix}=0
\eas
if \(i+j\neq p+k\).
We also have the induction relation
\bas
\begin{pmatrix} m&n&n+m-2p\\i&j+1&k+1\end{pmatrix}=
 \begin{pmatrix} m&n&n+m-2p\\i-1&j+1&k\end{pmatrix}
+\begin{pmatrix} m&n&n+m-2p\\i&j&k\end{pmatrix}.
\eas
\end{lem}
\begin{proof}
\bas
\Join^{m+n-2p}_{k+1} v^m\otimes  w^n &=& \Delta(N)  \Join^{m+n-2p}_k v^m\otimes  w^n  \\
 &=&
\sum_{i+j=p+k} \begin{pmatrix} m&n&n+m-2p\\i&j&k\end{pmatrix}  v_{i+1}^{m} \otimes v_{j}^{n}
\\&+& \sum_{i+j=p+k} \begin{pmatrix} m&n&n+m-2p\\i&j&k\end{pmatrix}  v_i^{m} \otimes v_{j+1}^{n}
 \\&=&
 \sum_{i+j=p+k} \begin{pmatrix} m&n&n+m-2p\\i-1&j+1&k\end{pmatrix}  v_{i}^{m} \otimes v_{j+1}^{n}
\\&+& \sum_{i+j=p+k} \begin{pmatrix} m&n&n+m-2p\\i&j&k\end{pmatrix}  v_i^{m} \otimes v_{j+1}^{n}
\eas
\end{proof}
\fi
\iffalse
\begin{lem}
The \(3j\)-symbols are orthogonal:
\bas
\lefteqn{\sum\begin{pmatrix} {m_1}& {n_1}& {m_1}+{n_1}-2p_1\\i_1&j_1& k_1\end{pmatrix}  
\begin{pmatrix} {m_2}& {n_2}& {m_2}+{n_2}-2p_2\\i_2&j_2& k_2\end{pmatrix} \binom{{m_1}}{i_1} \binom {{n_1}}{j_1}}&&
\\&=&
\delta_{k_1,k_2}\delta_{m_1,m_2}\delta_{n_1,n_2} \binom{m_1+n_1-2p_1}{k_1}
\|v^{m_1}\otimes w^{n_1}\|^2 \frac{\binom{m_1+n_1-p_1+1}{p_1}}{\binom{m_1}{p_1}\binom{n_1}{p_1}}
\eas
where the summation is over \(i_1+j_1=p_1+k_1=p_2+k_2=i_2+j_2.\)
\end{lem}
\begin{proof}
We compute \((\Join^{(m_1+n_1-2p_1)}_{k_1} v^{m_1}\otimes  w^{n_1},  \Join^{(m_2+n_2-2p_2)}_{k_2} v^{m_2}\otimes  w^{n_2} )_{V\otimes V}\).
\bas
\lefteqn{(\Join^{(m_1+n_1-2p_1)}_{k_1} v^{m_1}\otimes  w^{n_1} , \Join^{(m_2+n_2-2p_2)}_{k_2} v^{m_2}\otimes  w^{n_2} )_{V\otimes V}=}&&
\\&=&
\delta_{k_1,k_2} \binom{m_1+n_1-2p_1}{k_1}(\Join^{(m_1+n_1-2p_1)} v^{m_1}\otimes  w^{n_1} , \Join^{(m_2+n_2-2p_2)} v^{m_2}\otimes  w^{n_2} )_{\ker\Delta(M)}  
\\&=&
\delta_{k_1,k_2}\delta_{m_1,m_2}\delta_{n_1,n_2}  \binom{m_1+n_1-2p_1}{k_1}
\|v^{m_1}\otimes w^{n_1}\|^2 \frac{\binom{m_1+n_1-p_1+1}{p_1}}{\binom{m_1}{p_1}\binom{n_1}{p_1}}
\eas
\end{proof}
\fi
\iffalse
\begin{lem} 
One has \(\Delta(N)^\perp=\Delta(M)\) and \(\Delta(M)^\perp=\Delta(N)\), where \(\Delta(N)^\perp\) is the transpose of \(\Delta(N)\) with respect to the inner product \((\cdot,\cdot)_{V\otimes V}\):
\[
( \Delta(N) v , w )_{V\otimes V} =(v, \Delta(M)w)_{V\otimes V}, \quad v,w\in V\otimes V
\]
\end{lem}
\begin{proof}
\bas
(\Delta(N) v_{i_1}^{m_1}\otimes w_{i_2}^{m_2},v_{j_1}^{n_1}\otimes w_{j_2}^{n_2})&=&(v_{i_1+1}^{m_1}\otimes w_{i_2}^{m_2},v_{j_1}^{n_1}\otimes w_{j_2}^{n_2})+
(v_{i_1}^{m_1}\otimes w_{i_2+1}^{m_2},v_{j_1}^{n_1}\otimes w_{j_2}^{n_2})
\\&=&(v_{i_1+1}^{m_1},v_{j_1}^{n_1})(w_{i_2}^{m_2},w_{j_2}^{n_2})
+(v_{i_1}^{m_1},v_{j_1}^{n_1})(w_{i_2+1}^{m_2},w_{j_2}^{n_2})
\\&=&(v_{i_1}^{m_1},M v_{j_1}^{n_1})(w_{i_2}^{m_2},w_{j_2}^{n_2})
+(v_{i_1}^{m_1},v_{j_1}^{n_1})(w_{i_2}^{m_2},M w_{j_2}^{n_2})
\\&=&( v_{i_1}^{m_1}\otimes w_{i_2}^{m_2},\Delta(M) v_{j_1}^{n_1}\otimes w_{j_2}^{n_2})
\eas
\end{proof}
\fi
\iffalse
\section{Van der Waerden}
Van der Waerden \cite[\S 18, page\ 68]{vanderWaerden1932} uses the following notation:
\begin{itemize}
\item
his \(\mathfrak{D}_j\) (\(\rho_j\) in the English rewrite \cite{van2012group}) is our \(V_{2j}\).
\item
our \(M\) is his \(\hat{M}=x_2\frac{\partial}{\partial x_1}\), our \(N\) is his \(\hat{N}=x_1\frac{\partial}{\partial x_2}\)
\item
The groundform for \(V_m\) is in symbolic notation (cf \cite{olver1999classical}) \(G_u^m=(ux)^m=(u_1 x_1+u_2 x_2)^m\).
We identify  \(\binom{m}{j} u_1^{m-j}u_2^j\) with \(u_j^{(m)}\).
The inner product \((u_j^m,u_i^m)=\delta_{i,j} \binom{m}{i}\) corresponds to 
\bas
(u_1^{m-j}u_2^j,u_1^{m-i}u_2^i)&=&\frac{1}{\binom{m}{i}\binom{m}{j}} (u_j^m,u_i^m)=\frac{\delta_{i,j} \binom{m}{i}}{\binom{m}{i}\binom{m}{j}}
= \delta_{i,j} \frac{1}{\binom{m}{i}}.
\eas
\item 
his \((u_1x_1)^{j+m}(u_2x_2)^{j-m}\) is our \(u_{j-m}^{2j}\).
\item
his \(A=G_u^{2j}\Join^\lambda G_v^{2j^\prime}:=[uv]^\lambda(ux)^{2j-\lambda}(vx)^{2j^\prime-\lambda}=(u_1v_2-u_2v_1)^\lambda(u_1x_1+u_2x_2)^{2j-\lambda}(v_1x_1+v_2x_2)^{2j^\prime-\lambda}\)
corresponds to our 
\(\Join^{2j+2j^\prime-2\lambda} u^{2j}\otimes v^{2j^\prime}\) when evaluated at \(x_2=0\), that is, 
\bas
A_0&=&(u_1v_2-u_2v_1)^\lambda u_1^{2j-\lambda}v_1^{2j^\prime-\lambda}x_1^{2(j+j^\prime-\lambda)}
\\&=&\sum_{\nu=0}^\lambda (-1)^\nu \binom{\lambda}{\nu} (u_1v_2)^{\lambda-\nu} (u_2v_1)^\nu u_1^{2j-\lambda}v_1^{2j^\prime-\lambda}x_1^{2(j+j^\prime-\lambda)}
\\&=&\sum_{\nu=0}^\lambda (-1)^\nu \binom{\lambda}{\nu} u_1^{2j-\nu} u_2^{\nu} v_1^{\nu-\lambda +2j^\prime} v_2^{\lambda-\nu}\otimes  x_1^{2(j+j^\prime-\lambda)}
\\&=&\sum_{\nu=0}^\lambda (-1)^\nu \frac{\binom{\lambda}{\nu}}{\binom{2j}{\nu}\binom{2j^\prime}{\lambda-\nu}}  u_{\nu}^{(2j)} \otimes v_{\lambda-\nu}^{(2j^\prime)}\otimes  x_0^{(2j+2j^\prime-2\lambda)}
\eas
\item
our \(M\) is his \(x_2\frac{\partial}{\partial x_1}\), our \(N\) is his \(x_1\frac{\partial}{\partial x_2}\)
\item
We see that
\bas
A_k &=&\hat{N}^k A= (x_2\frac{\partial}{\partial x_1})^k A
\\&=&\frac{(2(j+j^\prime-\lambda))!}{(2(j+j^\prime-\lambda)-k))!}(u_1v_2-u_2v_1)^\lambda u_1^{2j-\lambda}v_1^{2j^\prime-\lambda}\otimes x_1^{2(j+j^\prime-\lambda)-k}x_2^k
\\&=&\frac{(2(j+j^\prime-\lambda))!}{(2(j+j^\prime-\lambda)-k))!}\sum_{\nu=0}^\lambda (-1)^\nu \binom{\lambda}{\nu} (u_1v_2)^{\lambda-\nu} (u_2v_1)^\nu  u_1^{2j-\lambda}v_1^{2j^\prime-\lambda}\otimes x_1^{2(j+j^\prime-\lambda)-k}x_2^k
\\&=&\frac{(2(j+j^\prime-\lambda))!}{(2(j+j^\prime-\lambda)-k))!}\sum_{\nu=0}^\lambda (-1)^\nu \binom{\lambda}{\nu} u_1^{-\nu+2j}u_2^{\nu} v_1^{\nu+2j^\prime-\lambda}v_2^{\lambda-\nu}\otimes x_1^{2(j+j^\prime-\lambda)-k}x_2^k
\\&=&\frac{(2(j+j^\prime-\lambda))!}{(2(j+j^\prime-\lambda)-k))!}\sum_{\nu=0}^\lambda (-1)^\nu \frac{\binom{\lambda}{\nu}}{\binom{2(j+j^\prime-\lambda)}{k}\binom{2j}{\nu}\binom{2j^\prime}{\lambda-\nu}} u_{\nu}^{(2j)} \otimes v_{\lambda-\nu}^{(2j^\prime)}\otimes x_k^{(2(j+j^\prime-\lambda))}
\\&=&\frac{(m+n-2p)!}{(m+n-p-k)!}\sum_{i+j=p} (-1)^i \frac{\binom{p}{i}}{\binom{m+n-2p}{k}\binom{m}{i}\binom{n}{j}} u_{i}^{(m)} \otimes v_{j}^{(n)}\otimes x_k^{(m+n-2p)}
\\&=&\frac{(m+n-2p-k)!}{(m+n-p-k)!}\sum_{i+j=p} (-1)^i \frac{p!k!(m-i)!(n-j)!}{m!n!} u_{i}^{(m)} \otimes v_{j}^{(n)}\otimes x_k^{(m+n-2p)}
\\&=&\frac{k!}{\binom{m+n-p-k}{p}}\sum_{i+j=p} (-1)^i \frac{(m-i)!(n-j)!}{m!n!} u_{i}^{(m)} \otimes v_{j}^{(n)}\otimes x_k^{(m+n-2p)}
\eas
\end{itemize}
\fi
\iffalse
\section{Koornwinder}
Translation of Koornwinder's paper \cite{koornwinder1981clebsch} to our notation.
\begin{itemize}
\item
\(\psi_n^l(x,y)=\binom{2l}{l-n} x^{l-n} y^{l+n}\). This corresponds to our \(\binom{2l}{l-n} v^{(2l)}_{l-n}=\binom{m}{i} v_i^{(m)}\).
\end{itemize}
\fi
\iffalse
\section{Structure constants for the 3D \(\mathcal{A}\)-family}
In this section we compute the \(P\)th transvectant of \(z^{m_1}\) and \(z^{m_2}\), that is \(\Join^{2{m_1}+2{m_2}-2P} z^{m_1}\otimes z^{m_2}\).
We know that this transvectant is in the kernel of \(M\) after contraction of the tensor product (since a tensor stays in the kernel of its arguments are switched and thus the symmetrized tensor is also in the kernel) and is therefore of a sum of monomials \(z^Q \Delta^R\).
Comparing the degrees we see that \({m_1}+{m_2}=Q+2R\), while comparing the \(H\) eigenvalues we see that \(2{m_1}+2{m_2}-2P=2Q\).
Thus we have \(Q={m_1}+{m_2}-P\) and \(2R={m_1}+{m_2}-({m_1}+{m_2}-P)=P\). This implies that \(P\) is even and we put \(P=2p\). Then \(p=R\) and we know that the transvectant is 
\( c z^{{m_1}+{m_2}-2p} \Delta^p\) if \(P\) is even and zero otherwise.
If we evaluate \( c z^{{m_1}+{m_2}-2p} \Delta^p\) for \(x=0\), we find \(c z^{{m_1}+{m_2}-2p} \Delta^p\equiv c (-1)^p z^{{m_1}+{m_2}-2p} y^{2p}\).
Evaluating at \(x=0\) means that we can compute with \(N_{app}=2y\frac{\partial}{\partial z}\) since the contribution of the \(x\frac{\partial}{\partial y}\)-term
ends up as zero anyway. Let \(v^{2{m_1}}=z^{m_1}\) and \(w^{2{m_2}}=z^{m_2}\). 
Recall the definition of the transvectant:
\bas
\Join^{m+n-2p}v^m \otimes w^{n}&=&
\sum_{i=0}^p (-1)^i \frac{\binom{p}{i}}{\binom{m}{i}\binom{n}{p-i}}  v_{i}^{(m)} \otimes w_{p-i}^{(n)}.
\eas
Then
\bas\label{T2}
                                \Join^{2{m_1}+2{m_2}-4p} z^{m_1}\otimes z^{m_2}&=&
                                \sum_{i=0}^{2p} (-1)^i \frac{\binom{2p}{i}}{\binom{2{m_1}}{i}\binom{2{m_2}}{2p-i}}  v_{i}^{(2{m_1})} \otimes w_{2p-i}^{(2{m_2})}
\\&=&
                                \sum_{i=0}^{2p} (-1)^i \frac{\binom{2p}{i}}{\binom{2{m_1}}{i}\binom{2{m_2}}{2p-i}}\frac{1}{i!(2p-i)!}  N^i z^{{m_1}} \otimes N^{2p-i}z^{{m_2}}
\\&\equiv&
                                \sum_{i=0}^{2p} (-1)^i \frac{\binom{2p}{i}}{\binom{2{m_1}}{i}\binom{2{m_2}}{2p-i}}\frac{1}{i!(2p-i)!}  N_{app}^i z^{{m_1}} \otimes N_{app}^{2p-i}z^{{m_2}}
\\&=&
                                \sum_{i=0}^{2p} (-1)^i 2^{2p}\frac{\binom{2p}{i}}{\binom{2{m_1}}{i}\binom{2{m_2}}{2p-i}}\frac{1}{i!(2p-i)!}  \frac{{m_1}!}{({m_1}-i)!} \frac{{m_2}!}{({m_2}-2p+i)!}y^{2p} z^{{m_2}+{m_1}-2p} 
\\&=&
                                \frac{{m_1}!{m_2}!(2p)!2^{2p}}{(2{m_1})!(2{m_2})!}\sum_{i=0}^{2p} (-1)^i \frac{(2{m_1}-i)!}{({m_1}-i)!} \frac{(2{m_2}-2p+i)! }{i! (2p-i)!({m_2}-2p+i)!}y^{2p} z^{{m_2}+{m_1}-2p} 
\\&\equiv&
{2}^{2\,p}\frac {{{m_1}+{m_2}-p\choose p}{{m_1}\choose p}{{m_2}\choose p}}{{2\,{m_1}\choose 2\,p}{2\,{m_2}\choose 2\,p}{2\,p \choose p}}{z}^{{m_1}+{m_2}-2\,p}{\Delta}^{p}.
\eas
\begin{rem}
There are two factors \((-1)^p\) involved here, one from the summation, the other from the relation \(y^2\mapsto -\Delta\).
\end{rem}
\fi
\iffalse
\begin{exm}
We recall the inversion formula:
\bas
v^{(m)}_i\otimes v^{(n)}_j&=&\sum_{p+k=i+j}\begin{pmatrix} m&n&m+n-2p\\i&j&k\end{pmatrix}\frac{ \binom{m}{i}\binom{n}{j}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes v^n.
\eas
Let \(r=i+j=p+k=1\).
Then 
\bas
v^{(m)}_1\otimes w^{(n)}_0&=&
\sum_{p+k=1}\begin{pmatrix} m&n&m+n-2p\\1&0&k\end{pmatrix}\frac{ m\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes w^n.
\\&=&
\begin{pmatrix} m&n&m+n-2\\1&0&0\end{pmatrix}\frac{ m^2n}{(m+n)}\Join^{(m+n-2)}v^m\otimes w^n.
\\&+&\begin{pmatrix} m&n&m+n\\1&0&1\end{pmatrix}\frac{ m}{(m+n)}\Join^{(m+n)}_{1}v^m\otimes w^n.
\eas
Recall  the definition of
the \(3j\)-symbol
\[\begin{pmatrix} m& n& m+n-2p\\i&j& k\end{pmatrix}=\sum_{f+g=k, g\leq i, f\leq j} (-1)^{i-k+f} \frac{\binom{p}{i-g}\binom{i}{g} \binom{j}{f}}{\binom{m}{i-g}\binom{n}{j-f}}, \quad i+j=p+k\]
which reduces to
\[\begin{pmatrix} m& n& m+n-2p\\1&0& k\end{pmatrix}=\sum_{g=k, g\leq i=1 } (-1)^{1-k} \frac{\binom{p}{1-k}\binom{1}{k} }{\binom{m}{1-k}}, \quad i+j=p+k\]
in our example.
We have
\[\begin{pmatrix} m& n& m+n-2\\1&0& 0\end{pmatrix}= - \frac{1}{m}, \]
\[\begin{pmatrix} m& n& m+n\\1&0& 1\end{pmatrix}=\sum_{f+g=1,g\leq i=1, f\leq j=0}  \frac{1 }{\binom{m}{0}}= 1,\]
Thus
\bas
v^{(m)}_1\otimes w^{(n)}_0&=&
\begin{pmatrix} m&n&m+n-2\\1&0&0\end{pmatrix}\frac{ m^2n}{(m+n)}\Join^{(m+n-2)}v^m\otimes w^n.
\\&+&\begin{pmatrix} m&n&m+n\\1&0&1\end{pmatrix}\frac{ m}{(m+n)}\Join^{(m+n)}_{1}v^m\otimes w^n.
\\&=&
-\frac{ mn}{(m+n)}\Join^{(m+n-2)}v^m\otimes w^n
+\frac{ m}{(m+n)}\Join^{(m+n)}_{1}v^m\otimes w^n.
\\&=&
-\frac{ mn}{(m+n)}(\frac{1}{n}  v^{(m)} \otimes w_{1}^{(n)}-\frac{1}{m}  v_{1}^{(m)} \otimes w^{(n)})
\\&+&\frac{ m}{(m+n)}(v^{(m)} \otimes w_{1}^{(n)}+v_{1}^{(m)} \otimes w^{(n)})
\\&=&
-\frac{ m}{(m+n)}  v^{(m)} \otimes w_{1}^{(n)}+\frac{ n}{(m+n)}  v_{1}^{(m)} \otimes w^{(n)}
\\&+&\frac{ m}{(m+n)}(v^{(m)} \otimes w_{1}^{(n)}+v_{1}^{(m)} \otimes w^{(n)})
\\&=&
v_{1}^{(m)} \otimes w^{(n)}.
\eas
\begin{thm}
Miracles happen!
\end{thm}
\end{exm}
\fi
\iffalse
We recall the inversion formula:
\bas
v^{(m)}_i\otimes w^{(n)}_j&=&\sum_{p+k=i+j}\begin{pmatrix} m&n&m+n-2p\\i&j&k\end{pmatrix}\frac{ \binom{m}{i}\binom{n}{j}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes w^n.
\eas
In this case this gives us a formula for \(N^{i_1} z^{\mu_1} \cdot N^{i_2} z^{\mu_2}\):
\bas
&&\frac{1}{{i_1}!{i_2}!} N^{i_1} z^{m_1} \cdot N^{i_2} z^{m_2}
\\&=&\sum_{2p+k={i_1}+{i_2}}\begin{pmatrix} 2{m_1}&2{m_2}&2{m_1}+2{m_2}-4p\\{i_1}&{i_2}&k\end{pmatrix}\frac{ \binom{2{m_1}}{{i_1}}\binom{2{m_2}}{{i_2}}\binom{2{m_1}}{2p}\binom{2{m_2}}{2p}}{\binom{2{m_1}+2{m_2}-4p}{k}\binom{2{m_1}+2{m_2}-2p+1}{2p}}\Join^{(2{m_1}+2{m_2}-4p)}_{k}v^{2{m_1}}\otimes v^{2{m_2}}
\\&=&\sum_{2p+k={i_1}+{i_2}}\begin{pmatrix} 2{m_1}&2{m_2}&2{m_1}+2{m_2}-4p\\{i_1}&{i_2}&k\end{pmatrix}\frac{ \binom{2{m_1}}{{i_1}}\binom{2{m_2}}{{i_2}}\binom{2{m_1}}{2p}\binom{2{m_2}}{2p}}{\binom{2{m_1}+2{m_2}-4p}{k}\binom{2{m_1}+2{m_2}-2p+1}{2p}}
%\Join^{(2{m_1}+2{m_2}-4p)}_{k}v^{2{m_1}}\otimes v^{2{m_2}}.
\\&\times&{2}^{2\,p}\frac{{m_1+m_2-p\choose p}{m_1\choose p}{m_2\choose p}}{{2\,{m_1}\choose 2\,p}{2\,{m_2}\choose 2\,p}{2\,p \choose p}}\frac{1}{k!} N^k {z}^{{m_1}+{m_2}-2\,p}{\Delta}^{p}.
\\&=&\sum_{2p+k={i_1}+{i_2}}\begin{pmatrix} 2{m_1}&2{m_2}&2{m_1}+2{m_2}-4p\\{i_1}&{i_2}&k\end{pmatrix}
\frac{ \binom{2{m_1}}{{i_1}}\binom{2{m_2}}{{i_2}}}{\binom{2{m_1}+2{m_2}-4p}{k}\binom{2{m_1}+2{m_2}-2p+1}{2p}\binom{2p}{p}}
%\Join^{(2{m_1}+2{m_2}-4p)}_{k}v^{2{m_1}}\otimes v^{2{m_2}}.
\\&\times&{2}^{2\,p}{m_1+m_2-p\choose p}{m_1\choose p}{m_2\choose p}\frac{1}{k!} N^k z^{{m_1}+{m_2}-2\,p}\Delta^{p}.
\eas
We define
\bas
\kappa^{i_1,m_1,n_1}_{i_2,m_2,n_2}&=&(i_1)!(i_2)!\sum_{2p+k={i_1}+{i_2}}\begin{pmatrix} 2{m_1}&2{m_2}&2{m_1}+2{m_2}-4p\\{i_1}&{i_2}&k\end{pmatrix}\frac{ \binom{2{m_1}}{{i_1}}\binom{2{m_2}}{{i_2}}}{\binom{2{m_1}+2{m_2}-4p}{k}\binom{2{m_1}+2{m_2}-2p+1}{2p}\binom{2p}{p}}
\\&\times&{2}^{2\,p}{m_1+m_2-p\choose p}{m_1\choose p}{m_2\choose p}\frac{1}{k!} 
\eas
Then 
\bas
N^{i_1} z^{m_1} \cdot N^{i_2} z^{m_2}&=& \sum_{2p+k={i_1}+{i_2}} \kappa^{i_1,m_1,n_1}_{i_2,m_2,n_2} N^k z^{{m_1}+{m_2}-2\,p}\Delta^{p}
\eas
Let us define \(v^{m+2n,2m}_k=\ad_N^k z^m \Delta^n E= (N^k z^m )\Delta^n E\), where \(E\) is the Euler operator.
Then
\bas
{[}v^{m_1+2n_1,2m_1}_{i_1},v^{m_2+2n_2,2m_2}_{i_2}{]}&=&(N^{i_1}z^{m_1})(N^{i_2} z^{m_2}) (m_1+2n_2-m_2-2n_2) \Delta^{n_1+n_2} E
\\&=& (m_1+2n_2-m_2-2n_2) \Delta^{n_1+n_2} \sum_{2p+k={i_1}+{i_2}} \kappa^{i_1,m_1,n_1}_{i_2,m_2,n_2} N^k z^{{m_1}+{m_2}-2\,p}\Delta^{p} E
\\&=& (m_1+2n_2-m_2-2n_2) \sum_{2p+k={i_1}+{i_2}} \kappa^{i_1,m_1,n_1}_{i_2,m_2,n_2} N^k z^{{m_1}+{m_2}-2\,p}\Delta^{n_1+n_2+p}E
\\&=& (m_1+2n_2-m_2-2n_2) \sum_{2p+k={i_1}+{i_2}} \kappa^{i_1,m_1,n_1}_{i_2,m_2,n_2} v_k^{{m_1}+{m_2}+2{n_1+2 n_2},2({m_1}+{m_2}-2\,p)} 
\eas
This gives us an equivariant decomposition with explicit structure constants (where explicit is a bit restricted by the \(3j\)-symbols, which are given as a finite sum).
%MARK
%\end{document}
\fi
\iffalse
Fa, can you verify the last \(\equiv\)?
\bas
\sum_{i=0}^{2p} {{\frac { \left( -1 \right) ^{i} \left( 2\,n \right) !\,p!\,q!\,
		\left( 2\,p-i \right) !\, \left( 2\,q-2\,n+i \right) !\,{2}^{2\,n}}{i
		!\, \left( 2\,n-i \right) !\, \left( 2\,p \right) !\, \left( 2\,q
		\right) !\, \left( p-i \right) !\, \left( q-2\,n+i \right) !}}}={\frac {{2}^{2\,n}{z}^{p+q-2\,n}{\Delta}^{n}{2
		\,n-p-q-1\choose n}{n-p-1\choose n}{n-q-1\choose n}}{{2\,p\choose 2\,n
	}{2\,q\choose 2\,n}{2\,n\choose n}}}
\eas
\bas
- \left( P+2 \right)  \left( -P+2\,N-1 \right)  \left( 2\,M-P-1
\right)  \left( 2\,M+2\,N-P \right) {{\it En}}^{2}- \left( -P+N+M
\right)  \left( M+N-P-1 \right)
\eas
\bas
&&
- \left( -P+N+M \right)  \left( M+N-P-1 \right) f \left( P \right) 
\\&&
-
\left( P+2 \right)  \left( 2\,N-P-1 \right)  \left( 2\,M-P-1 \right) 
\left( 2\,N+2\,M-P \right) f \left( P+2 \right) =0
\eas
\fi
\iffalse
We compute modulo \(x\), since \(x\) is \(N\)-invariant.
Then \(N^i z^p=\frac{p!}{(p-i)!} z^{p-i} y^i\).
\bas
                                (z^p,z^q)^{(2n)}
				&=&(2n)!\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
                                                \, \left( 2\,q-2n+i \right) !\,
                                        }{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
                                                !\,i!\, \left( 2\,q-2n \right) !}}{\rm N}^i(z^p)  { \rm N}^{2n-i}(z^q).
				\\&=&(2n)!\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
                                                \, \left( 2\,q-2n+i \right) !\,
                                        }{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
                                                !\,i!\, \left( 2\,q-2n \right) !}}\frac{p!}{(p-i)!} z^{p-i} y^i  \frac{q!}{(q-2n+i)!} z^{q-2n+i} y^{2n-i} 
				\\&=&(2n)!\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
                                                \, \left( 2\,q-2n+i \right) !\,
                                        }{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
                                                !\,i!\, \left( 2\,q-2n \right) !}}\frac{p!}{(p-i)!} z^{p+q-2n} y^{2n}  \frac{q!}{(q-2n+i)!} 
\eas
It follows that \bas
                                (z^p,z^q)^{(2n)}&=&z^{p+q-2n}\Delta^n(2n)!\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
                                                \, \left( 2\,q-2n+i \right) !\,
                                        }{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
                                                !\,i!\, \left( 2\,q-2n \right) !}}\frac{p!}{(p-i)!}  \frac{q!}{(q-2n+i)!}
\eas
\bas
&&\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
		\, \left( 2\,q-2n+i \right) !\,
	}{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
		!\,i!\, \left( 2\,q-2n \right) !}}\frac{p!}{(p-i)!}  \frac{q!}{(q-2n+i)!}
	\\
	&=&\left( n! \right) ^{2}{2\,n-p-q-1\choose n} {n-p-1\choose n}{n-q-1
	\choose n}
\eas
\fi
\section{Structure constants for the 3D \(\mathcal{A}\)-family}
In this section we compute the \(P\)th transvectant of \(z^{\mu_1}\) and \(z^{\mu_2}\), that is \(\Join^{2{\mu_1}+2{\mu_2}-2p} z^{\mu_1}\otimes z^{\mu_2}\).
\issue{FM}{check }
We know that this transvectant is in the kernel of \(M\) after contraction of the tensor product (since a tensor stays in the kernel of its arguments are switched and thus the symmetrized tensor is also in the kernel) and is therefore of a sum of monomials \(z^Q \Delta^R\), with \(\Delta=xz-y^2\).
Let \(m_i=2\mu_i, i=1,2\) be the \(H\)-eigenvalues of \(z^{\mu_i}\).
Comparing the degrees we see that \({\mu_1}+{\mu_2}=Q+2R\), while comparing the \(H\) eigenvalues we see that \({m_1}+{m_2}-2p=2Q\).
Thus we have \(Q={\mu_1}+{\mu_2}-p\) and \(2R=p\). This implies that \(p\) is even and we put \(p=2P\). Then \(P=R\) and we know that the transvectant is 
\( c z^{{\mu_1}+{\mu_2}-2P} \Delta^P\) if \(p\) is even and zero otherwise.
If we evaluate \( c z^{{\mu_1}+{\mu_2}-2P} \Delta^P\) for \(x=0\), we find \(c z^{{\mu_1}+{\mu_2}-2P} \Delta^p\equiv c (-1)^P z^{{\mu_1}+{\mu_2}-2P} y^{2P}\).
Evaluating at \(x=0\) means that we can compute with \(N_{app}=2y\frac{\partial}{\partial z}\) since the contribution of the \(x\frac{\partial}{\partial y}\)-term
ends up as zero anyway. Let \(v^{{m_1}}=z^{\mu_1}\) and \(w^{{m_2}}=z^{\mu_2}\). 
Recall the definition of the transvectant:
\bas
\Join^{m+n-2p}v^m \otimes w^{n}&=&
\sum_{i=0}^p (-1)^i \frac{\binom{p}{i}}{\binom{m}{i}\binom{n}{p-i}}  v_{i}^{(m)} \otimes w_{p-i}^{(n)}.
\eas
Then
\bas\label{T2}
                                \Join^{{m_1}+{m_2}-2p} z^{\mu_1}\otimes z^{\mu_2}&=&
                                \sum_{i=0}^{p} (-1)^i \frac{\binom{p}{i}}{\binom{{m_1}}{i}\binom{{m_2}}{p-i}}  v_{i}^{({m_1})} \otimes w_{p-i}^{({m_2})}
\\&=&
                                \sum_{i=0}^{p} (-1)^i \frac{\binom{p}{i}}{\binom{{m_1}}{i}\binom{{m_2}}{p-i}}\frac{1}{i!(p-i)!}  N^i z^{{\mu_1}} \otimes N^{p-i}z^{{\mu_2}}
\\&\equiv&
                                \sum_{i=0}^{p} (-1)^i \frac{\binom{p}{i}}{\binom{{m_1}}{i}\binom{{m_2}}{p-i}}\frac{1}{i!(p-i)!}  N_{app}^i z^{{\mu_1}} \otimes N_{app}^{p-i}z^{{\mu_2}}
\\&=&
                                \sum_{i=0}^{p} (-1)^i 2^{p}\frac{\binom{p}{i}}{\binom{{m_1}}{i}\binom{{m_2}}{p-i}}\frac{1}{i!(p-i)!}  \frac{{\mu_1}!}{({\mu_1}-i)!} \frac{{\mu_2}!}{({\mu_2}-p+i)!}y^{p} z^{{\mu_2}+{\mu_1}-p} 
\\&=&
                                \frac{{\mu_1}!{\mu_2}!(p)!2^{p}}{({m_1})!({m_2})!}\sum_{i=0}^{p} (-1)^i \frac{({m_1}-i)!}{({\mu_1}-i)!} \frac{({m_2}-p+i)! }{i! (p-i)!({\mu_2}-p+i)!}y^{p} z^{{\mu_1}+{\mu_2}-p} 
\\&\equiv&
{2}^{\,p}\frac {{{\mu_1}+{\mu_2}-P\choose P}{{\mu_1}\choose P}{{\mu_2}\choose P}}{{{m_1}\choose p}{{m_2}\choose p}{p \choose P}}{z}^{{\mu_1}+{\mu_2}-p}{\Delta}^{P}.
%\\&\equiv&
%{2}^{2\,p}\frac {{{m_1}+{m_2}-p\choose p}{{m_1}\choose p}{{m_2}\choose p}}{{2\,{m_1}\choose 2\,p}{2\,{m_2}\choose 2\,p}{2\,p \choose p}}{z}^{{m_1}+{m_2}-2\,p}{\Delta}^{p}.
\eas
\iffalse
\begin{rem}
Fa, what did Maple give as answer to 
\bas
                                &&\sum_{i=0}^{2p} (-1)^i \frac{(2{m_1}-i)!}{({m_1}-i)!} \frac{(2{m_2}-2p+i)! }{i! (2p-i)!({m_2}-2p+i)!}
                                \\
                                & =&
                                 (\frac{{m_1}!{m_2}!(2p)!}{(2{m_1})!(2{m_2})!})^{-1}\frac {{{m_1}+{m_2}-p\choose p}{{m_1}\choose p}{{m_2}\choose p}}{{2\,{m_1}\choose 2\,p}{2\,{m_2}\choose 2\,p}{2\,p \choose p}}
                                 \\&=&
                                 {\frac {M!\,N!\, \left( -1/2-N \right) !\, \left( -1/2-M \right) !\,{
                                 			16}^{-p}{-1+2\,p-N-M\choose -1/2+p-N}{2\,M\choose M}{2\,N\choose N}}{p
                                 		!\, \left( -1+p-M-N \right) !}}
                                 \eas
\end{rem}
\begin{rem}
There are two factors \((-1)^p\) involved here, one from the summation, the other from the relation \(y^2\mapsto -\Delta\).
\end{rem}
\fi
\iffalse
\begin{exm}
We recall the inversion formula:
\bas
v^{(m)}_i\otimes v^{(n)}_j&=&\sum_{p+k=i+j}\begin{pmatrix} m&n&m+n-2p\\i&j&k\end{pmatrix}\frac{ \binom{m}{i}\binom{n}{j}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes v^n.
\eas
Let \(r=i+j=p+k=1\).
Then 
\bas
v^{(m)}_1\otimes w^{(n)}_0&=&
\sum_{p+k=1}\begin{pmatrix} m&n&m+n-2p\\1&0&k\end{pmatrix}\frac{ m\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes w^n.
\\&=&
\begin{pmatrix} m&n&m+n-2\\1&0&0\end{pmatrix}\frac{ m^2n}{(m+n)}\Join^{(m+n-2)}v^m\otimes w^n.
\\&+&\begin{pmatrix} m&n&m+n\\1&0&1\end{pmatrix}\frac{ m}{(m+n)}\Join^{(m+n)}_{1}v^m\otimes w^n.
\eas
Recall  the definition of
the \(3j\)-symbol
\[\begin{pmatrix} m& n& m+n-2p\\i&j& k\end{pmatrix}=\sum_{f+g=k, g\leq i, f\leq j} (-1)^{i-k+f} \frac{\binom{p}{i-g}\binom{i}{g} \binom{j}{f}}{\binom{m}{i-g}\binom{n}{j-f}}, \quad i+j=p+k\]
which reduces to
\[\begin{pmatrix} m& n& m+n-2p\\1&0& k\end{pmatrix}=\sum_{g=k, g\leq i=1 } (-1)^{1-k} \frac{\binom{p}{1-k}\binom{1}{k} }{\binom{m}{1-k}}, \quad i+j=p+k\]
in our example.
We have
\[\begin{pmatrix} m& n& m+n-2\\1&0& 0\end{pmatrix}= - \frac{1}{m}, \]
\[\begin{pmatrix} m& n& m+n\\1&0& 1\end{pmatrix}=\sum_{f+g=1,g\leq i=1, f\leq j=0}  \frac{1 }{\binom{m}{0}}= 1,\]
Thus
\bas
v^{(m)}_1\otimes w^{(n)}_0&=&
\begin{pmatrix} m&n&m+n-2\\1&0&0\end{pmatrix}\frac{ m^2n}{(m+n)}\Join^{(m+n-2)}v^m\otimes w^n.
\\&+&\begin{pmatrix} m&n&m+n\\1&0&1\end{pmatrix}\frac{ m}{(m+n)}\Join^{(m+n)}_{1}v^m\otimes w^n.
\\&=&
-\frac{ mn}{(m+n)}\Join^{(m+n-2)}v^m\otimes w^n
+\frac{ m}{(m+n)}\Join^{(m+n)}_{1}v^m\otimes w^n.
\\&=&
-\frac{ mn}{(m+n)}(\frac{1}{n}  v^{(m)} \otimes w_{1}^{(n)}-\frac{1}{m}  v_{1}^{(m)} \otimes w^{(n)})
\\&+&\frac{ m}{(m+n)}(v^{(m)} \otimes w_{1}^{(n)}+v_{1}^{(m)} \otimes w^{(n)})
\\&=&
-\frac{ m}{(m+n)}  v^{(m)} \otimes w_{1}^{(n)}+\frac{ n}{(m+n)}  v_{1}^{(m)} \otimes w^{(n)}
\\&+&\frac{ m}{(m+n)}(v^{(m)} \otimes w_{1}^{(n)}+v_{1}^{(m)} \otimes w^{(n)})
\\&=&
v_{1}^{(m)} \otimes w^{(n)}.
\eas
\begin{thm}
Miracles happen!
\end{thm}
\end{exm}
\fi
We recall the inversion formula:
\bas
v^{(m)}_i\otimes w^{(n)}_j&=&\sum_{p+k=i+j}\begin{pmatrix} m&n&m+n-2p\\i&j&k\end{pmatrix}\frac{ \binom{m}{i}\binom{n}{j}\binom{m}{p}\binom{n}{p}}{\binom{m+n-2p}{k}\binom{m+n-p+1}{p}}\Join^{(m+n-2p)}_{k}v^m\otimes w^n.
\eas
In this case this gives us a formula for \(N^{i_1} z^{\mu_1} \cdot N^{i_2} z^{\mu_2}\):
\bas
&&\frac{1}{{i_1}!{i_2}!} N^{i_1} z^{\mu_1} \cdot N^{i_2} z^{\mu_2}
\\&=&\sum_{p+k={i_1}+{i_2}}\begin{pmatrix} {m_1}&{m_2}&{m_1}+{m_2}-2p\\{i_1}&{i_2}&k\end{pmatrix}\frac{ \binom{{m_1}}{{i_1}}\binom{{m_2}}{{i_2}}\binom{{m_1}}{p}\binom{{m_2}}{p}}{\binom{{m_1}+{m_2}-2p}{k}\binom{{m_1}+{m_2}-p+1}{p}}\Join^{({m_1}+{m_2}-2p)}_{k}v^{{m_1}}\otimes v^{{m_2}}
\\&=&\sum_{p+k={i_1}+{i_2}}\begin{pmatrix} {m_1}&{m_2}&{m_1}+{m_2}-2p\\{i_1}&{i_2}&k\end{pmatrix}\frac{ \binom{{m_1}}{{i_1}}\binom{{m_2}}{{i_2}}\binom{{m_1}}{p}\binom{{m_2}}{p}}{\binom{{m_1}+{m_2}-2p}{k}\binom{{m_1}+{m_2}-p+1}{p}}
%\Join^{(2{m_1}+2{m_2}-4p)}_{k}v^{2{m_1}}\otimes v^{2{m_2}}.
\\&\times&{2}^{2\,P}\frac{{\mu_1+\mu_2-P\choose P}{\mu_1\choose P}{\mu_2\choose P}}{{{m_1}\choose \,p}{{m_2}\choose p}{p \choose P}}\frac{1}{k!} N^k {z}^{{\mu_1}+{\mu_2}-p}{\Delta}^{P}.
\\&=&\sum_{p+k={i_1}+{i_2}}\begin{pmatrix} {m_1}&{m_2}&{m_1}+{m_2}-2p\\{i_1}&{i_2}&k\end{pmatrix}
\frac{ \binom{{m_1}}{{i_1}}\binom{{m_2}}{{i_2}}}{\binom{{m_1}+{m_2}-2p}{k}\binom{{m_1}+{m_2}-p+1}{2P}\binom{p}{P}}
%\Join^{(2{m_1}+2{m_2}-4P)}_{k}v^{2{m_1}}\otimes v^{2{m_2}}.
\\&\times&{2}^{p}{\mu_1+\mu_2-P\choose P}{\mu_1\choose P}{\mu_2\choose P}\frac{1}{k!} N^k z^{{\mu_1}+{\mu_2}-p}\Delta^{P}.
\eas
We define
\bas
\kappa^{i_1,\mu_1}_{i_2,\mu_2}(P)&=&\begin{pmatrix} {m_1}&{m_2}&{m_1}+{m_2}-2p\\{i_1}&{i_2}&i_1+i_2-p\end{pmatrix}\frac{ \binom{{m_1}}{{i_1}}\binom{{m_2}}{{i_2}}}{\binom{{m_1}+{m_2}-2p}{i_1+i_2-p}\binom{{m_1}+{m_2}-p+1}{p}\binom{p}{P}}
\\&\times&{2}^{p}{\mu_1+\mu_2-P\choose P}{\mu_1\choose P}{\mu_2\choose P}\frac{(i_1)!(i_2)!}{(i_1+i_2-p)!} .
\eas
\begin{rem}
This reduces, using Remark \ref{rem:pis0}, for \(P=0\) to
\bas
\kappa^{i_1,\mu_1}_{i_2,\mu_2}(0)&=&\begin{pmatrix} {m_1}&{m_2}&{m_1}+{m_2}\\{i_1}&{i_2}&i_1+i_2\end{pmatrix}\frac{ \binom{{m_1}}{{i_1}}\binom{{m_2}}{{i_2}}}{\binom{{m_1}+{m_2}}{i_1+i_2}\binom{i_1+i_2}{i_1}}
\\&=&
\frac{ \binom{{m_1}}{{i_1}}\binom{{m_2}}{{i_2}}}{\binom{{m_1}+{m_2}}{i_1+i_2}\binom{i_1+i_2}{i_1}}
=\frac{\binom{m_1+m_2-i_1-i_2}{m_1-i_1}}{\binom{m_1+m_2}{m_1}}.
%\\&=&
%\frac{i_1!i_2! m_1!m_2(i_1+i_2)!(m_1+m_2-i_1-i_2)!}{(i_1+i_2)!(m_1+m_2)!i_2!(m_2-i_2)! i_1!(m_1-i_1)!}
%\\&=&
%\frac{ m_1!m_2(m_1+m_2-i_1-i_2)!}{(m_1+m_2)!(m_2-i_2)! (m_1-i_1)!}
\eas
\end{rem}
Then 
\bas
N^{i_1} z^{\mu_1} \cdot N^{i_2} z^{\mu_2}&=& \sum_{p+k={i_1}+{i_2}} \kappa^{i_1,\mu_1}_{i_2,\mu_2}(P) N^k z^{{\mu_1}+{\mu_2}-p}\Delta^{P}
\eas
Let us define \(v^{\mu+2\nu,2\mu}_k=\sad_N^k z^\mu \Delta^\nu E= (N^k z^\mu )\Delta^\nu E\), where \(E\) is the Euler operator.
Then
\bas
{[}v^{\mu_1+2\nu_1,2\mu_1}_{i_1},v^{\mu_2+2\nu_2,2\mu_2}_{i_2}{]}&=&(N^{i_1}z^{\mu_1})(N^{i_2} z^{\mu_2}) (\mu_1+2\nu_1-\mu_2-2\nu_2) \Delta^{\nu_1+\nu_2} E
\\&=& (\mu_1+2\nu_1-\mu_2-2\nu_2) \Delta^{\nu_1+\nu_2} \sum_{p+k={i_1}+{i_2}} \kappa^{i_1,\mu_1+2\nu_1}_{i_2,\mu_2+2\nu_2}(P) N^k z^{{\mu_1}+{\mu_2}-p}\Delta^{P} E
\\&=& (\mu_1+2\nu_1-\mu_2-2\nu_2) \sum_{p+k={i_1}+{i_2}} \kappa^{i_1,\mu_1+2\nu_1}_{i_2,\mu_2+2\nu_2}(P) N^k z^{{\mu_1}+{\mu_2}-p}\Delta^{\nu_1+\nu_2+P}E
\\&=& (\mu_1+2\nu_1-\mu_2-2\nu_2) \sum_{p+k={i_1}+{i_2}} \kappa^{i_1,\mu_1+2\nu_1}_{i_2,\mu_2+2\nu_2}(P) v_k^{{\mu_1}+{\mu_2}+2{\nu_1+2 \nu_2},2({\mu_1}+{\mu_2}-p)} 
\eas
This gives us an equivariant decomposition with explicit structure constants (where explicit is a bit restricted by the \(3j\)-symbols, which are given as a finite sum).
Notice that if we choose to work \(\mod \Delta^{\nu_1+\nu_2+1}\), this reduces to
\bas
{[}v^{\mu_1+2\nu_1,2\mu_1}_{i_1},v^{\mu_2+2\nu_2,2\mu_2}_{i_2}{]}&=&(N^{i_1}z^{\mu_1})(N^{i_2} z^{\mu_2}) (\mu_1+2\nu_1-\mu_2-2\nu_2) \Delta^{\nu_1+\nu_2} E
\\&\equiv& (\mu_1+2\nu_1-\mu_2-2\nu_2) \Delta^{\nu_1+\nu_2}  \kappa^{i_1,\mu_1+2\nu_1}_{i_2,\mu_2+2\nu_2}(0) N^{i_1+i_2} z^{{\mu_1}+{\mu_2}} E \mod \Delta^{\nu_1+\nu_2+1}
\\&=& (\mu_1+2\nu_1-\mu_2-2\nu_2)  \kappa^{i_1,\mu_1+2\nu_1}_{i_2,\mu_2+2\nu_2}(0) N^{i_1+i_2} z^{{\mu_1}+{\mu_2}}\Delta^{\nu_1+\nu_2}E  \mod \Delta^{\nu_1+\nu_2+1}
\\&=& (\mu_1+2\nu_1-\mu_2-2\nu_2)  \kappa^{i_1,\mu_1+2\nu_1}_{i_2,\mu_2+2\nu_2}(0) v_{i_1+i_2}^{{\mu_1}+{\mu_2}+2{\nu_1+2 \nu_2},2({\mu_1}+{\mu_2})}  \mod \Delta^{\nu_1+\nu_2+1}
\eas
\iffalse
Fa, can you verify the last \(\equiv\)?
\bas
\sum_{i=0}^{2p} {{\frac { \left( -1 \right) ^{i} \left( 2\,n \right) !\,p!\,q!\,
		\left( 2\,p-i \right) !\, \left( 2\,q-2\,n+i \right) !\,{2}^{2\,n}}{i
		!\, \left( 2\,n-i \right) !\, \left( 2\,p \right) !\, \left( 2\,q
		\right) !\, \left( p-i \right) !\, \left( q-2\,n+i \right) !}}}={\frac {{2}^{2\,n}{z}^{p+q-2\,n}{\Delta}^{n}{2
		\,n-p-q-1\choose n}{n-p-1\choose n}{n-q-1\choose n}}{{2\,p\choose 2\,n
	}{2\,q\choose 2\,n}{2\,n\choose n}}}
\eas
\bas
- \left( P+2 \right)  \left( -P+2\,N-1 \right)  \left( 2\,M-P-1
\right)  \left( 2\,M+2\,N-P \right) {{\it En}}^{2}- \left( -P+N+M
\right)  \left( M+N-P-1 \right)
\eas
\bas
&&
- \left( -P+N+M \right)  \left( M+N-P-1 \right) f \left( P \right) 
\\&&
-
\left( P+2 \right)  \left( 2\,N-P-1 \right)  \left( 2\,M-P-1 \right) 
\left( 2\,N+2\,M-P \right) f \left( P+2 \right) =0
\eas
\fi
\iffalse
We compute modulo \(x\), since \(x\) is \(N\)-invariant.
Then \(N^i z^p=\frac{p!}{(p-i)!} z^{p-i} y^i\).
\bas
                                (z^p,z^q)^{(2n)}
				&=&(2n)!\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
                                                \, \left( 2\,q-2n+i \right) !\,
                                        }{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
                                                !\,i!\, \left( 2\,q-2n \right) !}}{\rm N}^i(z^p)  { \rm N}^{2n-i}(z^q).
				\\&=&(2n)!\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
                                                \, \left( 2\,q-2n+i \right) !\,
                                        }{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
                                                !\,i!\, \left( 2\,q-2n \right) !}}\frac{p!}{(p-i)!} z^{p-i} y^i  \frac{q!}{(q-2n+i)!} z^{q-2n+i} y^{2n-i} 
				\\&=&(2n)!\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
                                                \, \left( 2\,q-2n+i \right) !\,
                                        }{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
                                                !\,i!\, \left( 2\,q-2n \right) !}}\frac{p!}{(p-i)!} z^{p+q-2n} y^{2n}  \frac{q!}{(q-2n+i)!} 
\eas
It follows that \bas
                                (z^p,z^q)^{(2n)}&=&z^{p+q-2n}\Delta^n(2n)!\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
                                                \, \left( 2\,q-2n+i \right) !\,
                                        }{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
                                                !\,i!\, \left( 2\,q-2n \right) !}}\frac{p!}{(p-i)!}  \frac{q!}{(q-2n+i)!}
\eas
\bas
&&\sum _{i=0}^{2n}{\frac { \left( -1 \right) ^{i} \left( 2\,p-i \right) !
		\, \left( 2\,q-2n+i \right) !\,
	}{ \left( 2n-i \right) !\, \left( 2\,p-2n \right)
		!\,i!\, \left( 2\,q-2n \right) !}}\frac{p!}{(p-i)!}  \frac{q!}{(q-2n+i)!}
	\\
	&=&\left( n! \right) ^{2}{2\,n-p-q-1\choose n} {n-p-1\choose n}{n-q-1
	\choose n}
\eas
\fi
\bas
\eas

